Copositive Duality for Discrete Markets and Games

Optimization problems with discrete decisions are nonconvex and thus lack strong duality, which limits the usefulness of tools such as shadow prices and the KKT conditions. It was shown in Burer(2009) that mixed-binary quadratic programs can be written as completely positive programs, which are convex. Completely positive reformulations of discrete optimization problems therefore have strong duality if a constraint qualification is satisfied. We apply this perspective in two ways. First, we write unit commitment in power systems as a completely positive program, and use the dual copositive program to design a new pricing mechanism. Second, we reformulate integer programming games in terms of completely positive programming, and use the KKT conditions to solve for pure strategy Nash equilibria. To facilitate implementation, we also design a cutting plane algorithm for solving copositive programs exactly.

==> legacy_discontinued_content1_origin.tex <==
\section{Introduction}
{\cred Convex problems in economics, such as convex markets and games, often have unique properties, e.g., strong duality and fixed point theorem, which their nonconvex counterparts lack. Motivated by this perspective, many papers in the literature seek to connect nonconvex problems to convex problems. Some examples include studies of  markets with indivisible goods \citep{danilov2001discrete,baldwin2019understanding,tran2019product}, and nonconvex electricity markets \citep{o2005efficient}. Inspired by \cite{burer2009copositive} who transforms mixed-binary quadratic programs (MBQPs) to equivalent completely positive programs (CPPs), which are convex, we construct a notion of duality for mixed-integer programs (MIPs) and MBQPs via copositive programming. More specifically, we reformulate nonconvex economic problems, such as nonconvex markets and games containing binary decisions, with CPPs. This transformation enables us to work directly with the dual of a CPP, i.e., a copositive program (COP), and use properties such as strong duality and optimality conditions for those problems.} 

% Convex problems in economics, such as convex markets and convex games, often have unique properties, e.g., strong duality and fixed point theorem, that nonconvex problems lack. Motivated by this perspective, many papers in the literature seeks to connect nonconvex problems to convex problems. For example, \cite{danilov2001discrete}, \cite{baldwin2019understanding}, and \cite{tran2019product} which deal with nonconvex markets with indivisible goods prove that competitive equilibrium exists in such markets when demands satisfy ``discrete convexity", or equivalently the market problem can be formulated as a linear program that satisfies the unimodularity theorem. \cite{o2005efficient} fix the binary decisions in nonconvex electricity markets in order to linearly relax the optimization problem and obtain the shadow prices. Inspired by \cite{burer2009copositive} where the authors transform mixed-binary quadratic programs (MBQPs) to equivalent completely positive programs (CPPs), which are convex, we reformulate problems of nonconvex markets and games containing binary decisions with CPPs. This transformation enables us to work directly with the dual of a CPP, i.e. a copositive program (COP), and use properties such as strong duality and KKT conditions for those problems. {\cred In other words, we use copositive programming to construct a notion of duality for mixed-integer programs (MIP) and MBQPs.}

Copositive programming refers to linear programming over the convex cone of copositive matrices. The dual of a COP is a  CPP, which does the linear optimization over the cone of completely positive matrices. COPs and CPPs are both convex but NP-hard, and the latter has been shown to generalize MBQPs \citep{burer2009copositive,xu2018copositive}. While this does not point to a computational improvement, the convexity of COPs and CPPs offers new tools for analyzing MBQPs. In this paper, we leverage copositive duality in two major applications: pricing in discrete markets, and characterizing equilibria of integer programming games (IPGs). The presented ideas have potential to be applied in other nonconvex problems where discrete duality is useful. %, which motivates the transformation of nonconvex problems to convex problems via copositive programming in our work.

An immediate challenge in using copositive duality is that existing solution methods for COPs are either inexact, or require significant implementation/computational efforts. To address this issue, we design a novel cutting plane algorithm that exactly solves COPs when it terminates, which we employ in the two COP duality applications in this work. The algorithm consists of solving a sequence of MIPs only, hence is straightforward to implement and can benefit from advanced state-of-the-art MIP solvers. Moreover, it allows to have discrete variables by design, thus can be readily applied to mixed-integer programming over copositive matrices, which we henceforth refer to COPs with discrete variables. This feature is the first in the literature and useful for our IPG application. %Section \ref{subsec: bimatrix}. 


Our first application of copositive duality is unit commitment in power systems, in which the decision to turn a generator on or off is binary. It is commonly formulated as an MIP, for which efficient prices are difficult to construct; see,  e.g., \cite{liberopoulos2016critical}. We rewrite the MIP as a CPP, and use the dual COP to design a pricing mechanism based on shadow prices. The mechanism is budget balanced and, under certain conditions, individually rational. It is also straightforward to incorporate additional features, such as to enforce generator revenue adequacy, by adding constraints directly to the dual COP. This pricing mechanism has the potential to be generalized for other nonconvex markets, and provides a theoretical framework for analyzing such markets.

%Due to the lack of strong duality, nonconvex markets generally do not have shadow prices which leads to market equilibrium in convex markets. Our interest in nonconvex markets stems in particular from the energy market, where nonconvexity is introduced by binary commitment decisions of electricity generators. There is a large literature on the pricing of nonconvex energy markets, as summarized in the review paper by \cite{liberopoulos2016critical}. 

In our second application, we use copositive duality to characterize the Nash equilibria (NE) of IPGs with both binary and continuous decisions. There are well-known conditions guaranteeing the existence and uniqueness of NE in  convex (concave) games with convex strategy sets~\citep{debreu1952social,fan1952fixed, glicksberg1952further, rosen1965existence}. Also, due to the convexity of strategy sets, the Karush-Kuhn-Tucker (KKT) conditions can be used to compute the NE. We use copositive duality to extend some these results to IPGs, and use the KKT conditions to compute their equilibria. %, which include some classical games such as bimatrix games. 

% {\cred Below, we summarize our contributions. In the literature review of Section \ref{ch: lit_review} we will provide more details of these contributions:}

% (1) We use copositive programming to construct a notion of duality for MIPs and MBQPs. Such copositive duality is shown to be useful in major application problems including discrete markets and discrete games. It also has the potential to be applied in other nonconvex problems where discrete duality is useful.

% (2) We develop a novel cutting plane algorithm which exactly solves COPs when it terminates. The main advantage of our algorithm is that it is straightforward to implement as it only requires a MIP solver. {\cred In addition, it is the first algorithm that can handle COPs with both continuous and discrete variables}. With this cutting plane algorithm, we are able to solve COP formulations for nonconvex market pricing problems, as well as the {\cred mixed-integer} COP models for obtaining the NE of bimatrix games. 

% (3) We propose a new pricing scheme for nonconvex energy markets using copositive duality, which is proved to be revenue neutral. We also provide sufficient conditions for our pricing scheme to be individually rational. In addition we provide a modified version of our copositive duality-based pricing scheme which ensures revenue adequacy, and present numerical results comparing our pricing scheme with traditional ones from literature. Our pricing scheme has the potential to be generalized for other nonconvex markets, and provides a theoretical framework for analyzing nonconvex markets, as it has direct access to the dual pricing problem.

% (4) The literature on IPGs mainly focuses on algorithms of IPGs, with relatively limited theoretical developments, while we provide theoretical results for the existence and uniqueness of PNE in a special class of IPG called mixed-binary quadratic (MBQ) games, and formulate an optimization problem based on the KKT conditions for obtaining the PNE. In addition, for certain types of IPGs, we can reformulate its KKT conditions to a single COP problem, then solve it to obtain the NE.

%(3) We develop a novel cutting plane algorithm which exactly solves COPs when it terminates. The main advantage of our algorithm is that it is straightforward to implement as it only requires a MIP solver. With this cutting plane algorithm, we are able to solve COP formulations for nonconvex market pricing problems, as well as the COP models for obtaining the NE of bimatrix games. 

The reminder of the paper is organized as follows. In Section \ref{ch: lit_review} we review the literature on copositive programming, pricing in nonconvex markets, and discrete games. In Section \ref{ch: cop_duality} we %prove some useful results
provide the necessary background on CPPs and COPs. In Section \ref{ch: cut_plane} we present the new cutting plane algorithm for solving COPs. %, as well as some existing approximations for COP. 
In Section \ref{ch: app_pricing} we propose a COP-based pricing scheme for unit commitment, while in Section \ref{ch: app_game} we derive new results on the equilibria of IPGs. In Section \ref{ch: results} we illustrate the proposed ideas via computational experiments. We conclude the paper in Section \ref{sec:conc}.

{\cred We note that all the proofs in this paper are given in Section \ref{ec: proofs} of the e-companion.}

%---------------------%
\section{Literature Review}\label{ch: lit_review}
In this section, we review relevant papers and position our work in the literature to highlight its contributions. Section \ref{ch: review_cop} reviews the application of copositive programming in reformulating integer programs, and solution methods for COPs. Section \ref{ch: review_pricing} surveys the pricing schemes for nonconvex markets.  Section \ref{ch: review_game} focuses on the literature of integer programming games.%Finally, section \ref{ch: review_basic_cop} includes a concise introduction for copositive programming.Section \ref{ch: review_game} summarizes our contributions.
%-----%
\subsection{Copositive Programming}\label{ch: review_cop}
Copositive programming has been shown to generalize a number of NP-hard problems, such as quadratic optimization \citep{bomze2002solving}, two-stage adjustable robust optimization \citep{xu2018copositive, hanasusanto2018conic}, and MBQPs \citep{burer2009copositive}. In particular, \cite{burer2009copositive} shows that an MBQP is equivalent to a CPP. This reformulation is the basis of our work. %In Section \ref{ch: cop_duality} we extend \citep{burer2009copositive} to develop several useful results for the copositive reformulation of MBQPs, which becomes handy later in the paper. %The last example is particularly relevant to our work, as convert nonconvex market and game problems to convex problems, which is the basic idea of this work. 

At present, no industrial software can directly solve COPs. \cite{parrilo2000structured} constructs a hierarchy of semidefinite programs (SDPs), which is widely used to approximate COPs. For example, it is used by \cite{de2002approximation} %show that the COP model for calculating 
to find the stability number of a graph, and by %can be approximately solved via SDPs;
\cite{hanasusanto2018conic} %reformulates a
for two-stage distributionally robust linear programs.  % with a COP, and approximately solve the COP via SDPs. 
An exact algorithm for COPs based on simplicial partitions is proposed by \cite{bundfuss2009adaptive}. However, their algorithm is rather complex to implement. \cite{bomze2008new} and \cite{bomze2010copositivity} use cutting planes to strengthen the SDP relaxation for COPs, but both are problem specific and can only be used for quadratic programming and clique number problems, respectively. In this paper, we develop a novel cutting plane algorithm that exactly solves COPs when it terminates. Also, to the best of our knowledge, this is the first algorithm that can solve COPs with discrete variables.%The benefit of our cutting plane algorithm is that it is straightforward to understand, and only requires MIP solvers to implement. With this cutting plane algorithm, we are able to solve COP formulations for nonconvex market pricing problems, as well as the COP model for obtaining the PNE of bimatrix games. Recently, \cite{anstreicher2020testing} proposes a MIP model that checks whether a matrix is copositive, which provides a convenient way for separating non-copositive matrices. Based on this MIP model, w
%-----%
\subsection{Pricing in Discrete Markets}\label{ch: review_pricing}
Many markets have nonconvexities, e.g., due to binary decisions and indivisible goods. It is difficult to design a pricing mechanism in such markets because of the lack of strong duality. The pricing problem in those markets has been studied for decades. \cite{gale1984equilibrium} shows that a price equilibrium exists in a market where traders have at most one indivisible object. \cite{bevia1999buying} consider the pricing problem in economies with several types of indivisible goods. Recently, \cite{danilov2001discrete} and \cite{baldwin2019understanding} study the equilibrium in markets with indivisible goods via discrete convexity, or Unimodularity Theorem.


%Markets with nonconvexities (indivisibilities) have a large presence in the real world, with some of the examples include housing markets, and markets with investment or start-up/shut-down decisions. The pricing problem in such nonconvex markets has been studied for decades. Recently\cite{starr1969quasi} proves that when there are a large number of traders in the economy, the divergence from market equilibrium because of nonconvexity is negligible. By using a well-known result in combinatorial topology, \cite{gale1984equilibrium} shows that in a market where traders have at most one indivisible object, a price equilibrium exists under mild assumptions. \cite{bevia1999buying} consider the pricing problem in economies with several types of indivisible goods. \cite{danilov2001discrete} and \cite{baldwin2019understanding} propose a general existence theorem for equilibrium in markets with indivisible goods via discrete convexity, or Unimodularity Theorem. In this work, we develop a pricing scheme for electricity markets, which can be generalized to other markets with discrete decisions.  % \cite{scarf1994allocation} suggests that in markets with indivisibilities . 

A basic source of nonconvexity in electricity markets is the binary startup and shutdown decisions of generators. These decisions are optimized via unit commitment (UC), which is commonly formulated as an MIP \citep{carrion2006computationally}. The basic idea of most current approaches is to construct approximate shadow prices for the MIP. \cite{o2005efficient} eliminate the nonconvexity by fixing the binary decisions at their optimal values and pricing the resulting linear program (LP). We call this scheme restricted pricing (RP). RP and its variants are used by some independent system operators (ISOs) in the US, such as the Pennsylvania-New Jersey-Maryland Interconnect. However, RP is often too low to cover the costs of generators, in which uplift or make-whole payments are needed to ensure generator profitability. The  convex hull pricing (CHP) of \cite{hogan2003minimum} and \cite{gribik2007market} uses the Lagrangian multipliers of the demand constraints as prices, and has been shown shown to minimize uplift. A modified version of CHP called extended locational marginal pricing is used by the Midcontinent ISO. \cite{ruiz2012pricing} propose a primal-dual approach for pricing, which combines the UC problem and the dual of its linear relaxation, as well as revenue adequacy constraints that ensure nonnegative profit for each generator. We note that such revenue adequacy constraints eliminate uplift, but also modify the original UC problem and may therefore result in suboptimal decisions. 

We use the CPP reformulation of MBQP to design a new pricing scheme, which we refer to as copositive duality pricing (CDP). CDP is budget balanced, supports the optimal UC, and is flexible in that it provides direct access to the dual COP. We make use of this flexibility by adding a revenue adequacy constraint. We refer to the augmented pricing scheme as revenue-adequate CDP (RCDP). 

%In our work, our proposed copositive duality pricing (CDP) scheme provides prices that support the optimal UC solutions. In addition, {\cred our method provides direct access to the dual pricing problem, and thus is flexible enough to incorporate additional revenue adequacy constraints in the revenue adequate CDP (RCDP) scheme, to ensure that each generator is revenue adequate.} % Another approach to price electricity is called the {\it convex hull pricing (CHP)} \citep{hogan2003minimum, gribik2007market}. 

%Many works in nonconvex energy markets focus on finding a pricing scheme that has revenue adequacy, i.e. the price is sufficient to cover the cost, with minimum uplift costs. revenue adequacy, uniform / generator dependent price and uplift costs

%UC generally assumes a central planner's viewpoint, as it solves the operational problem for all generators in the system at the same time. Therefore,
It is desirable for a pricing scheme to ensure individual rationality, i.e., that individual generators have no incentive to deviate from the optimal UC solution. \cite{o2005efficient} prove that RP is individually rational. CHP satisfies individual rationality in some special cases, but in general it does not support each individual generator's profit-maximizing solution \citep{gribik2007market}. The primal-dual approach does not guarantee individual rationality either. 
%Our work uses a conic program for pricing. One example in the literature that uses similar tools is \cite{winnicki2019convex}, which studies the pricing problem of alternating current optimal power flow (ACOPF) problem with semidefinite cone constraints. They find that their pricing scheme is individually rational when the ACOPF problem has a zero duality gap. 
CDP does not in general lead to individual rationality, but we provide a simple sufficient condition under which it does.

Table \ref{tab:price_features} compares the properties of several pricing schemes, where ``$\circ$" indicates the existence of a sufficient condition in the literature for ensuring the property. For a more thorough review of pricing in nonconvex markets, we refer the reader to \citep{liberopoulos2016critical}.
\begin{table}[h]
\centering
\caption{Features of Pricing Schems}
\label{tab:price_features}
\begin{tabular}{lccc}
\hline
\multicolumn{1}{c}{} & Uplift & Optimal & Individual  \\
Scheme               & free  & UC      & rationality \\ \hline
RP                  & $\times$    & $\checkmark$     & $\checkmark$         \\
CHP                  & $\times$    & $\times$      & $\circ$          \\
Primal-dual          & $\checkmark$    & $\times$      & $\times$          \\
CDP                  & $\times$    & $\checkmark$     & $\circ$     \\
RCDP         & $\checkmark$     & $\times$     & $\times$         \\ \hline
\end{tabular}
\end{table}
%{\cgreen (Cheng: \cite{azizan2020optimal}, which was recently published on OR, claims in their literature review (Table 1) that CHP supports competitive equilibrium, which means it ensures individual rationality, among other things. However, \cite{gribik2007market} says that only under special assumptions will CHP support competitive equilibrium. So is \cite{azizan2020optimal} wrong?)}
%-----%
\subsection{Integer Programming Games}\label{ch: review_game}
IPGs are a class of games where each player's action set contains integer decisions. Some applications of IPGs include bimatrix games, Nash-Cournot energy production games \citep{gabriel2013solving}, and Cournot game with indivisible goods \citep{kostreva1993combinatorial}. IPGs are also referred to as ``games with at least one player solving a combinatorial optimization problem" \citep{kostreva1993combinatorial}, and ``games with discrete strategy sets" \citep{sagratella2016computing}. Most papers in this field focus on algorithms that finds NE, and they are only applicable on IPGs with only integer decisions \citep{koppe2011rational, sagratella2016computing, carvalho2017computing}. Theoretical works are relatively sparse, including \citep{mallick2011existence} and \citep{sagratella2016computing}, which respectively provide NE existence conditions for two-person discrete games and 2-groups partitionable discrete games. In this work we provide conditions for the existence and uniqueness of pure NE (PNE) in IPGs with both continuous and discrete variables, as well as KKT conditions for obtaining the PNE. 
%\cite{koppe2011rational} propose a generating functions-based method for computing the PNE of IPGs with only integer decisions. \cite{mallick2011existence} identifies conditions for the existence of PNE in a special type of IPG, namely the two-person discrete games. \cite{sagratella2016computing} presents a branching method for computing the whole solution set of Nash equilibria in IPGs with only integer decisions, and also provide the existence condition for the NE of a special type of IPG called the 2-groups partitionable discrete NE problem. \cite{carvalho2017computing} develop a sampled generation method, which finds the NE when the IPG contains only integer decisions, and finds an $\epsilon$-equilibrium NE for IPGs with both integer and continuous variables. In general, the literature on IPGs is on the algorithmic side, while {\cred we provide conditions for the existence and uniqueness of PNE, as well as KKT conditions for obtaining the PNE.}
%with relatively limited theoretical developments, while in this work we provide theoretical results for the existence of NE in a class of IPGs called mixed-binary quadratic (MBQ) games, and formulate an optimization problem based on the KKT conditions for obtaining the NE. %study n-player noncooperative MBQ games, where the strategy set contains both binary and continuous variables, and the payoff functions can be either linear or quadratic. We

Similar to our approach, in the literature there are several applications of convex optimization to IPGs. \cite{parrilo2006polynomial} reformulate zero-sum polynomial games as a single SDP. \cite{ahmadi2020semidefinite} use SDP to find the additive $\epsilon$-approximate NE of bimatrix games. Closely related to our work, \cite{sayin2019optimal} study a Stackelberg game with binary decisions in the context of optimal hierarchical signaling. They reformulate each player's optimization problem as a CPP, and solve the CPP and its dual COP approximately with SDP. Our work differs from the above in that we analyze the equilibria of general IPGs, and for certain classes we can obtain the PNE by solving a single COP exactly.

%we can reformulate its KKT conditions to a single COP problem, and solve for the NE exactly with our proposed cutting plane algorithm. 
%------------------%
%\cite{azizan2020optimal} propose a pricing framework for nonconvex markets with general nonconvex costs. They also compare the proposed pricing scheme with other commonly used nonconvex market pricing schemes in the energy market literature, and conclude that their pricing scheme can obtain smaller total payments and uplift costs. However, the authors claim that the revenue from total payments should be minimized and match the total costs, while in traditional market equilibrium it is common to observe positive profits. For example, in convex markets, only the marginal producer's cost will equal to the shadow price, while the costs of non-marginal producers are smaller than the shadow price, earning them positive suppliers' surpluses. This type of positive profits are needed for paying off the costs of raising capital \citep{borenstein_2019}. Therefore, making the suppliers' surplus zero by forcing payment equal to costs can distort the market. Also, the model proposed by \cite{azizan2020optimal} can not be solved exactly. In our paper, we propose a pricing scheme which first lift the nonconvex optimization problem to a convex completely positive program, then obtain the traditional shadow price from this convex reformulation. In addition, we propose a novel algorithm to exactly solve the convex pricing problem

%\hrule
%Market equilibrium and optimization algorithms:
%
%\cite{chen2007note} proposes convex programming models for some general types of Fisher market and mixed Fisher and Arrow-Debreu market.
%
%\cite{devanur2008market} proposes the first polynomial time algorithm that uses the primal-dual method and KKT conditions to compute a Fisher market equilbrium.

%\hrule
%Markets with discrete goods:
%
%\cite{hassidim2011non} finds that for markets with indivisible goods, there always exists mix-strategy Nash Equilibrium, even under cases where price-based equilibrium does not exist.
%
%\cite{budish2011combinatorial} (a JPE paper) proposes a new mechanism for combinatorial assignment problem. (the following are from Wikipedia ``Fisher Market") It studied the most general setting in which agents can have arbitrary preference relations over bundles. He invented the mechanism of Approximate Competitive Equilibrium from Equal Incomes, which relaxes the CEEI conditions in two ways: (1) The agents' incomes are not exactly equal, and (2) a small number of items may remain unallocated. He proved that an approximate-CEEI always exists (although Othman et al[12] recently proved that the computation of approximate-CEEI is PPAD complete).
%
%\cite{babaioff2017competitive} (the following are from Wikipedia) studied whether CE exists when the incomes are generic, i.e., do not satisfy a finite set of equalities. In other words: whether there exists a CE for almost all income-vectors. They proved existence for three goods, and for four goods and two agents. They proved non-existence for five goods and two agents. Later, it has proved that with four goods and three agents, CE may not exist when the valuations are non-additive, but always exists when the valuations are additive.
%
%\cite{sayin2019optimal} 
%
%\hrule
%Application of IPG:
%
%\cite{bompard2006micro} models the competitive electricity market as a Cournot game.

%---------------------%
\section{Background}\label{ch: cop_duality}
In this section, we define CPP and COP and state some basic results. %Section \ref{ch: preliminary} contains a brief introduction to copositive programming. Section \ref{ch: new_results} presents some new results we derive for the CPP reformulation of MBQPs.%In the application problems of this work, we need to reformulate the MBQP problem with CPP, and then obtain the dual COP problem to get useful results. Therefore, in this section 
Throughout the paper, we use bold letters for vectors. $\tr(\cdot)$ denotes the trace of a matrix and $(\cdot)^\top$ denotes the transpose of a vector or matrix.
%-----%
\subsection{Preliminaries}\label{ch: preliminary}
%We first review some basic concepts in copositive programming that are relevant to our work. %{\cred \sout{For a more complete introduction to copositive programming, we refer the readers to the review papers of \cite{dur2010copositive} and \cite{bomze2012copositive}.}}

Let $\mc{S}_n$ be the set of $n$-dimensional real symmetric matrices. The copositive cone $\mc{C}_n$ is defined as:
\begin{align}\label{eq: def_cop}
\mc{C}_n=\left\{X\in\mc{S}_n\;|\; \mathbf{y}^\top X \mathbf{y} \geq0\textrm{ for all } \mathbf{y}\in\mathbb{R}^n_+\right\}.
\end{align}
%If we have strict inequality in \eqref{eq: def_cop}, then $X$ is strictly copositive and $X\in \interior(\mc{C}_n)$, where $\interior(\mc{C}_n)$ represents the interior of $\mc{C}_n$.
The dual cone of $\mc{C}_n$ is the completely positive cone $\mc{C}_n^*$:
\begin{align}\label{eq: def_cpp}
\mc{C}_n^*=\left\{XX^\top \;|\; X\in\mb{R}^{n\times r}_+ \right\}.
\end{align}
%If $X$ is entrywise strictly positive, then $XX^\top\in \interior(\mc{C}_n^*)$ \citep{groetzner2018factorization}.

In COP (CPP), we optimize a linear function of the matrix $X$ subject to linear constraints and $X\in\mc{C}_n$ ($X\in\mc{C}_n^*$).
%has a linear objective, linear constraints, and the con is an optimization problem defined over the copositive matrix $X\in\mc{C}_n$, with objective and constraints linear in $X$. Similarly, a (linear) CPP, which is the dual of COP, is an optimization problem defined over $X\in\mc{C}_n^*$ with objective and constraints linear in $X$.
Because COP and CPP are convex, strong duality holds if one of the certain regularity conditions is satisfied, e.g., Slater's condition, which requires the feasible region of either COP or CPP to have an interior point.
%----%
\subsection{CPP Reformulation of MBQP} \label{ch: new_results}
In this section, we state the two CPP reformulations of MBQP given in \cite{burer2009copositive}. We also derive their COP duals.

%In this section, we state some useful results on COP and CPP. We first present the dual COP problem for the CPP reformulation. Then we give a CPP reformulation that is slightly different than the CPP reformulations in \cite{burer2009copositive}. Moreover, we prove some useful results on the relationship of solutions from MBQP and its CPP reformulation.

Consider the MBQP:
\begin{subequations}\label{eq: bqp}
\begin{alignat}{4}
\mc{P}^\bqp: \min ~~&\x^\top Q \x + 2\c \x~~ \label{eq: bqp_obj}\\
\st ~~&\ajtop\x = b_j &&\forall j = 1, ..., m\label{eq: bqp_1}\\
&x_k\in \{0,1\} &&\forall k\in\mc{B}\label{eq: bqp_2}\\
&{\bf x} \in \mb{R}^n_+ \label{eq: bqp_3}
\end{alignat}
\end{subequations}
where $\mc{B}\subseteq\{1,...,n\}$ is the set of indices for the binary elements of $\x$. Without loss of generality we assume the matrix $Q$ is symmetric.

\cite{burer2009copositive} gives two CPP reformulations of $\mc{P}^\bqp$, (C) and (C'), which here we refer to as $\mc{P}_o^\cpp$ and  $\mc{P}_r^\cpp$, where ``$o$" and ``$r$" subscripts indicate original and reformulation, respectively. The original formulation is obtained by squaring the linear constraints and introducing the matrix of variables for the bilinear expressions:
\begin{subequations}\label{eq: cpp_origin}
\begin{alignat}{4}
\mc{P}_o^\cpp : \min ~~&\tr(Q X) + 2\c {\bf x}\label{eq: cpp_origin_obj}\\
\st ~~& \ajtop{\bf x} = b_j &&\forall j = 1, ..., m\label{eq: cpp_origin_1}\\
& \ajtop X \aj = b_j^{2} &&\forall j = 1, ..., m.\label{eq: cpp_origin_2}\\
& x_k = X_{kk} &&\forall k\in\mc{B}\label{eq: cpp_origin_3}\\
&\left[\begin{array}{cc}
1 & {\bf x}^\top \\
{\bf x} & X
\end{array}\right]\in\mc{C}_{n+1}^*.\label{eq: cpp_origin_5}
\end{alignat}
\end{subequations}
%we call the reformulation $\mc{P}_o^\cpp$ the original CPP reformulation in the following text.

We now derive the dual of \eqref{eq: cpp_origin}. For convenience, define:
\begin{align}\label{eq: define_vars}
Y = \left[\begin{array}{cc}
1 & {\bf x}^\top \\
{\bf x} & X
\end{array}\right]; \
\tilde{Q}=\left[
\begin{array}{cc}
0&  \bm{0}^{1\times n} \\
\bm{0}^{n\times 1}& Q
\end{array}
\right]; \
C=\left[
\begin{array}{cc}
0& \c \\
\mathbf{c} & \bm{0}^{n\times n}
\end{array}
\right]; \
A_j = \left[
\begin{array}{cc}
0& 1/2 \ajtop \\
1/2 \aj & \bm{0}^{n\times n}
\end{array}
\right],\ \forall j=1,...,m.
\end{align}
%and 
%\begin{align*}
%A_j = \left[
%\begin{array}{cc}
%0& 1/2 \ajtop \\
%1/2 \aj & \bm{0}^{n\times n}
%\end{array}
%\right],\quad j=1,...,m
%\end{align*}
We also define the matrices $\tilde{A}_j = [0, \ajtop]^\top[0, \ajtop], \forall j = 1,...,m$, as well as for each $k\in\mc{B}$ the matrix $B_k$ with entries
%Let numbers in brackets $[\cdot] ([\cdot, \cdot])$ denote the index (indices) of a vector (matrix). Define 
%For $k\in\mc{B}$, define
%\begin{align*}
%\tilde{A}_j [l_1, l_2]=\left\{\begin{array}{ll}
%\aj[l_1 - 1]\aj[l_2 - 1] &\text{if}~ 2\leq l_1, l_2 \leq n + 1, \\
%0 & \textrm{otherwise}
%\end{array}\right.
%\end{align*}
%and $B_k$, $k\in\mc{B}$, such that
\begin{align*}
(B_k)_{l_1,l_2}=\left\{\begin{array}{ll}
1/2 & \textrm{if } l_1=k+1,\; l_2=1~\text{or}~l_1=1,\; l_2=k+1\\
-1 & \textrm{if } l_1=k+1,\; l_2=k+1\\
0 & \textrm{otherwise}
\end{array}\right..
\end{align*}%1/2 & \textrm{if } l_1=1,\; l_2=k+1\\
Then, $\mc{P}_o^\cpp$ can be written as
\begin{subequations}\label{eq: cpp_origin_lifted}
\begin{alignat}{4}
\min \quad& \textrm{Tr}(\tilde{Q} Y) + \textrm{Tr}(C Y)\label{eq: cpp_origin_lifted_obj}\\
\st \quad& \textrm{Tr}(A_j Y)=b_j\quad \forall j=1,...,m\label{eq: cpp_origin_lifted_1}\\
&\textrm{Tr}(\tilde{A}_j Y)=b_j^2 \quad \forall j=1,...,m\label{eq: cpp_origin_lifted_2}\\
&\textrm{Tr}(B_k Y)=0\quad \forall k\in\mc{B}\label{eq: cpp_origin_lifted_3}\\
&Y\in\mc{C}_{n+1}^*.\label{eq: cpp_origin_lifted_4}
\end{alignat} 
\end{subequations}

Let $\pmb{\gamma}^o$, $\pmb{\beta}^o$, $\pmb{\delta}^o$,and $\Omega^o$ be the respective dual variables of constraints \eqref{eq: cpp_origin_lifted_1} - \eqref{eq: cpp_origin_lifted_4}. The dual of $\mc{P}_o^\cpp$ is the following COP:
\begin{subequations}\label{eq: cop_origin}
\begin{alignat}{4}
\mc{P}_o^\cop : \max_{\pmb\gamma^o,\pmb\beta^o,\pmb\delta^o,\Omega^o} \quad&\sum_{j=1}^m\Big(\gamma^o_j b_j+\beta^o_j b_j^2\Big) \label{eq: cop_origin_obj}\\
\st \quad & \tilde{Q} + C - \sum_{j = 1}^m \gamma^o_j A_j - \sum_{j = 1}^m \beta^o_j \tilde{A}_j - \sum_{k\in\mc{B}}\delta^o_k B_k - \Omega^o = 0\label{eq: cop_origin_2}\\
& \Omega^o \in\mc{C}_{n+1}.\label{eq: cop_origin_3}
\end{alignat}
\end{subequations}
%where $\mc{C}$ is a cone of copositive matrices as defined in \eqref{eq: def_cop}.

\cite{burer2009copositive} shows that $\mc{P}^\bqp$ and $\mc{P}_o^\cpp$ are equivalent, in the sense that (i) $\opt(\mc{P}^\bqp) = \opt(\mc{P}_o^\cpp)$, where $\opt(\cdot)$ is the optimal objective value; and (ii) if $(\xstar, X^*)$ is optimal for $\mc{P}_o^\cpp$, then $\mathbf{x}^*$ is in the convex hull of optimal solutions of $\mc{P}^\bqp$. The second point indicates that $\mathbf{x}^*$ is not necessarily feasible for $\mc{P}^\bqp$, i.e., it is possible for some $x_k^*$ with $k\in\mc{B}$ to be fractional. Regarding the optimal solutions, we have the following useful observations: %More specifically, we summarize the relationship between the optimal solutions of $\mc{P}^\bqp$ and $\mc{P}_o^\cpp$ in the following two remarks: %However, if $\xstar$ is feasible for $\mc{P}^\bqp$, and  $Q \succeq 0$, then $\xstar$ is an optimal solution to $\mc{P}^\bqp$,  as shown in the following proposition: %Notice that the equivalence between $\mc{P}^\bqp$ and $\mc{P}_r^\cpp$ means 

%=== Proposition ====%
\begin{remark}\label{th: feas_bqp_x}
Let $(\xstar, X^*)$ be an optimal solution for $\mc{P}_o^\cpp$. If $Q\succeq 0$ and $\xstar$ is feasible for $\mc{P}^\bqp$, then $\xstar$ is an optimal solution of $\mc{P}^\bqp$.
\end{remark}
%Proofs in this paper are given in  Section \ref{ec: proofs} of the e-companion.
%=== End of Proposition ====%

%Conversely, for the optimal solution of $\mc{P}^\bqp$, $\x^*$, then $(\x^*, \x^* \x^{*\top})$ is optimal for $\mc{P}_o^\cpp$, as shown in Proposition \ref{th: qip_sol}:
%=== Proposition ====%
\begin{remark}\label{th: qip_sol}
If $\xstar$ is an optimal solution to $\mc{P}^\bqp$, then $(\xstar, \xstar \mathbf{x}^{*\top})$ is optimal to $\mc{P}_o^\cpp$. %, where $X^*_i = \xstari \mathbf{x}^{*\top}_i$.  %{\cgreen (This theorem might have been proved in some other literature. But I cannot find anything right now. -- Cheng)}
\end{remark}
%=== End of Proposition ====%

%====ANOTHER PROOF OF THIS PROPOSITION!====
%=== Proposition ====%
%\begin{proposition}\label{th: qip_sol}
%Given an optimal solution to $\mc{P}^\bqp$, $\x^*$, there exists an optimal solution $(\x^*, X^*)$ to $\mc{P}^{\textrm{CPP}}$, where $X^* = \x^* \x^{*\top}$.  %{\cgreen (This theorem might have been proved in some other literature. But I cannot find anything right now. -- Cheng)}
%\end{proposition}
%
%\proof{Proof.}
%Denote the feasible region of $\mc{P}^\bqp$ as $\text{Feas}(\mc{P}^\bqp)$, and the feasible region of $\mc{P}^{\text{CPP}}$ as $\text{Feas}(\mc{P}^{\text{CPP}})$. Also, define
%\begin{align*}
%&\text{Feas}^+(\mc{P}^\bqp) := \conv\Bigl\{\begin{pmatrix} 1 \\ \x \end{pmatrix} \begin{pmatrix}1 \\ \x \end{pmatrix}^\top  : \x \in \text{Feas}(\mc{P}^\bqp)\Bigr\}\\
%&\text{Feas}^+(\mc{P}_r^\cpp) := \Bigl\{\begin{pmatrix} 1 & \x^\top  \\ \x & X\end{pmatrix} : (\x, X) \in \text{Feas}(\mc{P}_r^\cpp)\Bigr\}.
%\end{align*}
%For an optimal solution of $\mc{P}^\bqp$, $\x^*$, we have $\x^* \in \text{Feas}(\mc{P}^\bqp)$. Therefore, $\begin{pmatrix} 1 \\ \x^* \end{pmatrix} \begin{pmatrix}1 \\ \x^* \end{pmatrix}^\top  = \begin{pmatrix} 1 & \x^{*\top} \\ \x^* & \x^* \x^{*\top}\end{pmatrix} \in \text{Feas}^+(\mc{P}^\bqp)$.
%
%According to the Proposition 2.1 in \cite{burer2009copositive}, $\text{Feas}^+(\mc{P}^\bqp)\subseteq \text{Feas}^+(\mc{P}_r^\cpp)$. Thus, $\begin{pmatrix} 1 & \x^{*\top} \\ \x^* & \x^* \x^{*\top}\end{pmatrix} \in \text{Feas}^+(\mc{P}_r^\cpp)$. By definition, this means $(\x^*, \x^* \x^{*\top}) \in \text{Feas}(\mc{P}_r^\cpp)$. 
%
%It remains to prove that the feasible solution $(\x^*, \x^* \x^{*\top})$ is also optimal for $\mc{P}_r^\cpp$. Notice that the corresponding objective value of the solution $(\x^*, \x^* \x^{*\top})$ is $\tr(Q \x^* \x^{*\top}) + c^\top  \x^*$, which equals the optimal solution of $\mc{P}^\bqp$. Since the optimal values of $\mc{P}^\bqp$ and $\mc{P}_r^\cpp$ are equivalent, $\tr(Q \x^* \x^{*\top}) +  c^\top  \x^*$ is also the optimal value of $\mc{P}_r^\cpp$ . Therefore, the solution $(\x^*, \x^* \x^{*\top})$ is both feasible and optimal to $\mc{P}_r^\cpp$.
%\Halmos\endproof
%=== End of Proposition ====%
%The same result holds for the CPP reformulation $\mc{P}_o^\cpp$, because of the equivalence between $\mc{P}_o^\cpp$ and $\mc{P}_r^\cpp$. As we will need this result in the following sections, we formally write it in Lemma \ref{th: qip_sol2}:
%\begin{lemma}\label{th: qip_sol2}
%Given an optimal solution to $\mc{P}^\bqp$, $\x^*$, there exists an optimal solution $(\x^*, X^*)$ to $\mc{P}_o^\cpp$, where $X^* = \x^* \x^{*\top}$.  
%\end{lemma}
%--new cpp reform---
We also make use of the second CPP reformulation given in \cite{burer2009copositive}, $\mc{P}_r^\cpp$ (in Section \ref{ch: app_game}). The advantages of $\mc{P}_r^\cpp$ over $\mc{P}_o^\cpp$ are that (i) it has a smaller dimensional cone constraint, $X\in\mc{C}_n^*$, which may improve computational efficiency, and (ii) it may have an interior, whereas $\mc{P}_o^\cpp$ never does. $\mc{P}_r^\cpp$ is a valid reformulation of $\mc{P}^\bqp$ if the following Key Property is satisfied:
%Next, we propose a CPP reformulation for $\mc{P}^\bqp$ that is slightly different from CPP models ($C$) (i.e. our model \eqref{eq: cpp_origin}) and ($C'$) (i.e. the model \eqref{eq: cpp_projected} below) of \cite{burer2009copositive}. {\cred This new reformulation makes some of our subsequent proofs in Sections \ref{ch: app_game} more straightforward, because it contains constraints \eqref{eq: bqp_1} in their original linear form, and requires only $X$ to be completely positive in the conic constraint.} We provide this CPP reformulation in Proposition \ref{th: reform}:
%\begin{proposition} \label{th: reform}
%Assume problem $\mc{P}^\bqp$ satisfies the following assumption:
\begin{align}\label{a: alpha}
\tag{KP} \exists\; \mathbf{y}\in\mb{R}^{m}~~\st \sum^m_{j=1}y_j \aj \geq 0,\; \sum^{m}_{j=1} y_j b_j = 1.
\end{align}
Setting ${\pmb\alpha} := \sum^m_{j=1}y_j\aj $, the CPP is obtained as:
\begin{subequations}\label{eq: cpp_reform}
\begin{alignat}{4}
\mc{P}_r^\cpp : \min ~~& \tr(Q X) + 2\c \x \label{eq: cpp_obj}\\
\st ~~& \ajtop{\bf x} = b_j &&\forall j = 1, ..., m\label{eq: cpp_1}\\
& \ajtop X \aj = b_j^{2} &&\forall j = 1, ..., m\label{eq: cpp_2}\\
& x_k = X_{kk} &&\forall k\in\mc{B}\label{eq: cpp_3}\\
&{\cred x_l = \tr(\frac{\pmb\alpha \eltop + \el \pmb\alpha^\top}{2} X)}&~~& \forall l = 1,...,n\label{eq: cpp_4}\\
%&{\bf x} \in \mb{R}_+^{l}\label{eq: cpp_game_5}\\
& X\in\mc{C}_n^*.\label{eq: cpp_5}
\end{alignat}
\end{subequations}

Note that $\mc{P}_r^\cpp$, as written above, looks slightly different from (C') in \cite{burer2009copositive}. This is because we have included the variable ${\mathbf x}$ via the constraint ${\mathbf x}=X\alpha$, and made several corresponding substitutions. This makes the proofs in Section \ref{ch: app_game} more straightforward. {\cred Note that we write the constraint ${\mathbf x}=X\alpha$ in the symmetric form of \eqref{eq: cpp_3}, otherwise taking the dual of a CPP with non-symmetric linear constraints will bring extra complications (see a detailed discussion of this in Section \ref{} of e-companion).} Also note that Remarks \ref{th: feas_bqp_x} and \ref{th: qip_sol} straightforwardly extend to $\mc{P}_r^\cpp$.

% \begin{remark}
Condition \eqref{a: alpha} is usually not restrictive. For example, if $\mc{P}^\bqp$ contains or implies a constraint of the form $\sum_{i\in\mc{I}}a_i x_i = b$, where $a_i\geq 0$, $i\in\mc{I}$, and $b>0$, and this is the $\ell^{\text{th}}$ constraint of $\mc{P}^\bqp$, then we can construct a valid $\y$ with $1/b$ in the $\ell^{\text{th}}$ entry and 0 elsewhere.
% \end{remark}

%{\it Remark 2.} It is proved in \cite{burer2009copositive} that reformulation $\mc{P}_o^\cpp$ does not have any interior points. Thus, $\mc{P}_o^\cpp$ does not satisfy Slater's condition for strong duality. On the other hand, $\mc{P}_r^\cpp$ may have interior points. %In addition, compared with $\mc{P}_o^\cpp$ and reformulation \eqref{eq: cpp_projected}, the reformulation $\mc{P}_r^\cpp$ makes some of our subsequent proofs in Sections \ref{ch: app_game} more straightforward, because it contains constraints \eqref{eq: bqp_1} in their original linear form, and requires only $X$ to be completely positive in the conic constraint.

% \begin{remark}
Despite its lack of an interior, $\mc{P}_o^\cpp$ may be useful because (i) it does not require \eqref{a: alpha} to hold, {\cgreen (Maybe get rid of this) (ii) $\mc{P}_r^\cpp$ may need additional constraints to enforce symmetry in numerical implementations, which we discuss in the next section,} and (iii) strong duality may still hold, which we often observe in our numerical examples.
% \end{remark}


%{\it Remark 3.} Despite the lack of interior point, $\mc{P}_o^\cpp$ and its dual $\mc{P}_o^\cop$ can still be useful because:
%
%(i) They do not require the property \eqref{a: alpha}.
%
%{\cred (ii) $\mc{P}_r^\cpp$ may require more constraints to ensure symmetry of X. For more details please see our discussion in Section \ref{ch: cut_plane}.}
%{\cred \sout{(ii) $\mc{P}_o^\cop$ can have better computational performance than $\mc{P}^\cop$. When solving the dual COP problem, both our proposed cutting plane algorithm and SDP solvers require the matrix in the conic constraint to be symmetric. $\mc{P}_o^\cop$ naturally satisfies this requirement, as the symmetry of matrices $\tilde{Q}$, C, $A_j$, $\tilde{A}_j$, and $B_k$ ensures the symmetry of $\Omega$ in \eqref{eq: cop_origin_3}. For $\mc{P}^\cop$, however, symmetry of $\Omega$ is generally not guaranteed. This can be addressed by adding extra constraints in $\mc{P}_r^\cpp$ to ensure the symmetry of $X$. Those extra constraints in $\mc{P}_r^\cpp$ relaxes the dual, $\mc{P}^\cop$, and can lead to a worse computational performance compared with $\mc{P}_o^\cop$. For more details on the symmetry of COP, see Section \ref{subch: symmetry_cop}.}}

%(iii) Slater's condition is not a necessary condition for strong duality. We observe that in our experiments, strong duality holds for $\mc{P}_o^\cpp$ in some instances despite the lack of Slater's condition.

%{\cred As $\mc{P}_r^\cpp$ is also equivalent to $\mc{P}^\bqp$, we can easily extend the properties of problem $\mc{P}_o^\cpp$, i.e. Properties \ref{th: feas_bqp_x} and \ref{th: qip_sol}, to problem $\mc{P}_r^\cpp$.}

Finally, we write the dual of $\mc{P}_r^\cpp$. Let $\pmb{\gamma}$, $\pmb{\beta}$, $\pmb{\delta}$, $\pmb{\xi}$, and $\Omega$ be the respective dual variables of constraints \eqref{eq: cpp_1} - \eqref{eq: cpp_5}. The dual of $\mc{P}_r^\cpp$ is the COP: {\cgreen (Cheng: Could be removed, along with the discussion on symmetry, if we need more space.)}
\begin{subequations}\label{eq: cop}
\begin{alignat}{4}
\mc{P}_r^\cop : \max_{\pmb\gamma,\pmb\beta,\pmb\delta,\pmb\xi, \Omega} \quad&\sum_{j=1}^m\Big(\gamma_j b_j+\beta_j b_j^2\Big) \label{eq: cop_obj}\\
\st \quad&2\mathbf{c}-\sum_{j=1}^m \gamma_j \aj -\sum_{k\in\mc{B}}\delta_k \ek - {\cred \sum_{l=1}^n \xi_l \el} = {\mathbf 0}\label{eq: cop_1} \\
& Q - \sum_{j = 1}^m \beta_j \aj \ajtop + \sum_{k\in\mc{B}}\delta_k \ek \ektop + {\cred \sum^n_{l=1} \xi_l \frac{\pmb\alpha \eltop + \el \pmb\alpha^\top}{2}} - \Omega = 0\label{eq: cop_2}\\
& \Omega\in\mc{C}_n \label{eq: cop_3}
\end{alignat}
\end{subequations}
where $\ek\in\mb{R}^n$ is the $k^{\text{th}}$ unit  vector. % with 1 in the $k^{\textrm{th}}$ entry and 0 elsewhere.%---------------------%
\section{Cutting plane algorithm}\label{ch: cut_plane}
%\section{Solution Methods for COP}\label{ch: solution_algo}
To make use of copositive duality, we must be able to solve COPs. At present, no industrial solver can handle COPs. In the literature they are often approximately solved via SDPs (see Section \ref{ec: sdp_approx} of the e-companion). To solve COPs exactly, we design a novel cutting plane algorithm, which returns the optimal solution when it terminates. % In Section \ref{ch: approx_dual} we first review the SDP approximations for COPs from literature. In Section \ref{ch: cut_plane}, Section \ref{subch: symmetry_cop} includes an implementation note when algorithms for COP require the COP cone to be symmetric.
%Sections \ref{subch: algo_cpp} and \ref{ch: approx_dual} respectively review the SDP approximations for CPPs and COPs in the literature. 
%To obtain the electricity prices in Section \ref{ch: app_pricing}, we need to either solve the dual of CPP reformulation \eqref{eq: uc1_cpp1}, which is a COP, or solve the CPP \eqref{eq: uc1_cpp1} directly and obtain its optimal dual solutions. Also, to solve the KKT conditions in Section \ref{ch: kkt_special_2}, we need to solve a COP. 
%----%
%\subsection{SDP Approximations of COPs}\label{subch: approx_dual}
%----%
%\subsection{A Novel Cutting Plane Algorithm for COP}\label{ch: cut_plane}

The cutting plane algorithm is applicable for the following general type of COPs with mixed-integer linear constraints over a copositive cone:%The dual problem $\mc{P}^\cop$ is a COP. As we mentioned in the Introduction section, there are very few algorithms available to solve COPs. 
\begin{subequations}\label{eq: general_cop}
\begin{alignat}{4}
\max~~ &\mathbf{q}^{\top} \pmb\lambda + \tr(H^{\top} \Omega)\\
\st ~~&\mathbf{d}^\top \pmb\lambda + \tr(D_i^{\top} \Omega) = g_i &~~~&\forall i = 1,...,m\\
&\pmb\lambda\geq \boldsymbol{0}\\
&\Omega\in \mc{C}_{n_c}\label{eq: general_cop_4}\\
& \lambda_k \in \mb{Z} &~~~& \forall k\in\mc{L}
\end{alignat}
\end{subequations}
where $\pmb\lambda$ is an $n_l$-dimensional vector, $\mc{L}$ is the index set for integer variables in $\pmb\lambda$, $\Omega\in\mb{R}^{n_c \times n_c}$. $\mc{C}_{n_c}$ is an $n_c$-dimensional copositive cone. Notice that the COP problems $\mc{P}_o^\cop$ \eqref{eq: cop_origin} and $\mc{P}_r^\cop$ \eqref{eq: cop} are special cases of the COP \eqref{eq: general_cop}. 

The algorithm starts with relaxing \eqref{eq: general_cop} by removing the conic constraint \eqref{eq: general_cop_4} to obtain the initial master problem, which is iteratively refined with the addition of cuts. At each iteration, we solve the master problem to obtain an optimal solution  denoted by $(\bar{\pmb\lambda}, \bar{\Omega})$. To decide whether $\bar{\Omega}$ is copositive, we employ the MIP problem proposed by \cite{anstreicher2020testing}, which checks copositivity based on a recent characterization of copositive matrices that uses the concept of ``almost copositivity" \citep{dickinson2019new}. This MIP problem serves as the separation problem, i.e., the subproblem, in our cutting plane algorithm: 
%Our cutting plane algorithm is based on the following result from \citep{anstreicher2020testing}. Consider the MIP:
\begin{subequations}\label{eq: separation}
\begin{alignat}{4}
\SP(\Omega): \ \max~~&w\\
\st ~~&\Omega \mathbf{z} \leq -w\mathbf{1} + M^\top (1- \mathbf{u})\label{eq: separation_b}\\
&\mathbf{1}^\top \mathbf{u}\geq q\label{eq: separation_c}\\
& w\geq 0\\
& \mathbf{0}\leq \mathbf{z}\leq \mathbf{u}\\
& \mathbf{u}\in\{0,1\}^{n_c}
\end{alignat}
\end{subequations}
where $q = 1$ (or can be chosen as a larger integer depending on problem structure), $\mathbf{1}$ is a vector of all ones, and $M \in \mb{R}^{n_c\times n_c}_{++}$ is a matrix of large numbers. By Theorem 2 of  \cite{anstreicher2020testing}, $\bar{\Omega}$ is copositive if and only if the optimal objective of SP is zero.

%In words, the algorithm proceeds by solving \eqref{eq: general_cop} without the copositivity constraint, \eqref{eq: general_cop_4}; this is a relaxation. We test whether the relaxed solution, $\Omega$, is copositive via \SP. If yes
At any iteration, if the optimal value of the subproblem is zero, then the master problem solution is feasible and optimal for the COP \eqref{eq: general_cop}. Otherwise, as $\bar{\Omega}$ is not copositive, we add the following cut to the master problem:%, and repeat:
\begin{align}\label{eq: cop_cut}
\mathbf{\bar{z}}^\top \Omega \mathbf{\bar{z}}\geq 0
\end{align}
where $\mathbf{\bar{z}}$ is an optimal solution of \SP($\bar{\Omega}$). 

Note that the cut \eqref{eq: cop_cut} does not eliminate any feasible solutions from \eqref{eq: general_cop}. This is because for any $\mathbf{\bar{z}}\in\mb{R}^{n_c}_+$, any copositive matrix $\Omega$ satisfies $\mathbf{\bar{z}}^\top \Omega \mathbf{\bar{z}}\geq 0$. Moreover, as desired, it removes the candidate master problem solutions infeasible to the COP:

%This removes $\bar{\Omega}$ from the feasible set of the relaxation. %The full algorithm is given in Algorithm \ref{algo: cutting_planes}.

%$\bar{w}=0$, where $\bar{w}$ is the optimal solution for $w$ and equals the optimal objective value of \eqref{eq: separation}.

%If the separation problem suggests that $\hat{\Omega}$ is copositive, then we can conclude that $(\hat{\lambda}, \hat{\Omega})$ is optimal to the original COP problem \eqref{eq: general_cop}. Otherwise, let $\mathbf{\bar{z}}$ be the optimal value of $\mathbf{z}$ in problem \eqref{eq: separation}, we add the following {\it cut} to the relaxed problem to eliminate $\hat{\Omega}$ from its feasible region:
%\begin{align}\label{eq: cop_cut}
%\mathbf{\bar{z}}^\top \Omega %\mathbf{\bar{z}}\geq 0
%\end{align}
%and re-solve the relaxed problem. 

%Theorem \ref{th: cop_cut} we show that the cut \eqref{eq: cop_cut} removes the infeasible solution, $X$. %$\hat{\Omega}$.

\begin{proposition}\label{th: cop_cut}
If the optimal value of \SP($\bar{\Omega}$) %the separation problem \eqref{eq: separation} 
is nonzero, then \eqref{eq: cop_cut} cuts off $\bar{\Omega}$. %from the feasible set.
\end{proposition}
%Proofs in this paper are given in  Section \ref{ec: proofs} of the e-companion.

\begin{comment}
We use \MP to denote the {\it master problem}, i.e., the relaxed problem where the conic constraint in \eqref{eq: general_cop} is replaced with a set of cuts in the form of \eqref{eq: cop_cut}. We use $\{cuts\}$ to denote the set of cuts in (MP). The complete algorithm is as follows.
%To make the algorithm more clear, we write out the relaxed problem \eqref{eq: general_cop} where the conic constraints are replaced by a set of cuts, which is conventionally named as the {\it master problem}:
%\begin{subequations}\label{eq: master}
%\begin{alignat}{4}
%\MP : \max~~ &\mathbf{c}^{l\top} \pmb\lambda + \tr(C^{c\top} \Omega)\\
%\st ~~&\ail \pmb\lambda + \tr(A_i^{c\top} \Omega) = d_i &~&i = 1,...,m\\
%&\pmb\lambda\geq 0\\
%& x_k \in \mb{Z} &~~~& k\in\mc{B}\\
%&\{cuts\}
%\end{alignat}
%\end{subequations}
%where $\{cuts\}$ is a set of cuts in the form of \eqref{eq: cop_cut}, which are added iteratively into the master problem.

%====Algorithm===
\begin{algorithm}[H]\label{algo: cutting_planes}
\SetAlgoLined
%\KwResult{Write here the result }
 {\bf Initialization}: Set k = 0, $\{cuts\} = \emptyset$\;
 Solve \MP to obtain an initial solution $\hat{\Omega}^0$\;
 Solve \SP with $\Omega = \hat{\Omega}^0$ and obtain optimal solutions $\bar{w}$ and $\mathbf{\bar{z}}$\;
 \While{$\bar{w} > 0$}{
   $\{cuts\} = \{cuts\}\cup\{\mathbf{\bar{z}}^\top \Omega \mathbf{\bar{z}}\geq 0\}$\;
   $k = k + 1$\;
   Solve \MP to obtain an initial solution $\hat{\Omega}^k$\;
   Solve \SP with $\Omega = \hat{\Omega}^k$ and update optimal solutions $\bar{w}$ and $\mathbf{\bar{z}}$\;
%  \eIf{condition}{
%   instructions1\;
%   instructions2\;
%   }{
%   instructions3\;
%  }
 }
 \caption{Cutting plane algorithm for COP}
\end{algorithm}
\end{comment}
%======
Since \SP~is an MIP, we can strengthen its LP relaxation to improve its computational efficiency. \cite{anstreicher2020testing} suggests doing so by setting $M_{ik} = 1 + \sum_{j = 1, ~j\neq i}^{n_c}\{\bar{\Omega}_{ij}: \bar{\Omega}_{ij} > 0\}, \forall k = 1,...,n_c$. Another way to strengthen the separation problem is to let $q = 2$. \SP~will still be a valid problem with $q=2$ if $\diag(\hat{\Omega}) \geq 0$ \citep{anstreicher2020testing}. Luckily, $\diag(\bar{\Omega}) \geq 0$ is always valid for the original COP \eqref{eq: general_cop} because $\Omega\in\mc{C}_{n_c}$. Therefore, we can add the constraint $\diag(\bar{\Omega}) \geq 0$ to the intial master problem and increase the value of $q$ to 2 in \SP.

In some cases the master problem is unbounded at initialization. There are several methods to deal with this. One method is to impose a large constant as the bound for elements of $\Omega$. When the algorithm %\ref{algo: cutting_planes} 
terminates, gradually relax and eventually remove these bounds but keep all the added cuts, and continue the algorithm until it terminates again. 
In our COP duality applications, there is an easier way to judge if the first termination reaches optimality. Because in the COP duality framework the original MBQP problem \eqref{eq: bqp} is usually easy to solve, we can compare the optimal objective of MBQP with the optimal objective at the first termination when solving COP (we still want to solve the dual COP problem even if we have solved the MBQP, because COP solutions have practical meanings). If those two objectives are equivalent, then because of strong duality the COP solution at the first termination is already optimal. 
%In the context of our application, where the COP is obtained from the CPP reformulation of a MBQP, there is an easier way to judge if the first termination reaches optimality: compare the optimal result at the first termination with the optimal result of the original MBQP problem \eqref{eq: bqp}. If they are equivalent then because of strong duality this solution is optimal. %add a regularization term in the objective of (MP):

Using the optimal solution from the original MBQP problem \eqref{eq: bqp} problem, $x^*$, another way to bound \MP at initialization is to add the complementary slackness constraint $\tr(x^*x^{*\top} \Omega) = 0$. This constraint is valid when strong duality holds for the problem. Therefore, if the algorithm %\ref{algo: cutting_planes} 
terminates at a solution where strong duality does not hold, then the solution obtained with the additional complementary slackness constraint may not be valid. 

We could not prove that the cutting plane algorithm %\ref{algo: cutting_planes} 
can terminate in finite steps. However, in our numerical experiments, the algorithm converges well. Moreover, in our electricity market pricing application, we observe that the COP solution values corresponding to revenue and profit get stabilized over time. Therefore, we can still use the solution even if the algorithm does not converge when it hits the iteration limit (see Section \ref{subsec: electricity_markets_results}).
%If it does not terminate, we cannot evaluate the quality of master problem solution, because even a small nonzero value of $\bar{w}$ still means $\hat{\Omega}$ violates the conic constraint.

%{\cgreen (Add description on the termination condition: $w < 1e4$ or $|zYz) < 1e4$ or $iteration > 500 rounds$)} 
%----%
%\subsection{Enforcing Symmetry for COP Cones}\label{subch: symmetry_cop}
{\cred An implementation detail that is worth noting is that the cutting plane algorithm requires the conic constraint to be symmetric. }However, enforcing symmetry on $\Omega$ in the dual formulation \eqref{eq: cop} may cause infeasibility, as the CPP reformulation $\mc{P}_r^\cpp$ \eqref{eq: cpp_reform} does not ensure the symmetry of $X$. Therefore, to solve dual formulation $\mc{P}_r^\cop$ \eqref{eq: cop}, we need to rewrite constraint \eqref{eq: cop_2} in a different form. More specifically,  we add additional constraints $X_{ij} = X_{ji},\forall i<j, i,j = 1,...,m$ to \eqref{eq: cpp_reform}. Let $\pi_{ij}, \forall i<j, i,j = 1,...,m$ denote the dual variables correspond to those extra constraints, then the dual problem \eqref{eq: cop} will be relaxed, with constraint \eqref{eq: cop_2} being replaced by the following constraint containing $\pi_{ij}$:
\[Q - \sum_{j = 1}^m \beta_j \aj \ajtop + \sum_{k\in\mc{B}}\delta_k \ek \ektop + \sum_{i=1}^{m-1}\sum_{j=i+1}^m\pi_{ij}(\mathbf{e}_i \mathbf{e}_{j}^\top - \mathbf{e}_j \mathbf{e}_{i}^\top) + \pmb\alpha \pmb\xi^\top - \Omega = 0. \]
%---------------------%
\section{Pricing unit commitment}\label{ch: app_pricing}
In this section we use copositive duality to design a pricing mechanism for UC. UC optimally schedules the startups and shutdowns of the generators in a power system, typically over a 48 hour horizon. The problem is usually formulated as an MIP, in which the startup and shutdown decisions are binary variables. We reformulate the MIP as a CPP in Section \ref{subch: uc_reform}, and use the dual to define prices in Section \ref{subch: pricing_mechanism}, which we modify in Section \ref{subch: mod_cop_pricing} to guarantee revenue adequacy for individual generators.

%This problem is usually solved for a {\it day-ahead} market, which decides the operation schedule of the following day. The nonconvexity of this day-ahead energy market comes from the binary start-up/shut-down decisions. We obtain the electricity prices by first reformulating the MIP UC problem to a CPP (Section \ref{subch: uc_reform}), then derive the optimal dual values for some constraints in the CPP reformulation and set them as prices (Section \ref{subch: pricing_mechanism}). We also prove that under some assumptions this set of prices are revenue neutral and individually rational. Additionally, in Section \ref{subch: mod_cop_pricing} we propose a modified version of our pricing scheme that ensures revenue adequacy for individual generators.

Let $\mc{G}$ be the set of generators and $\mc{T}$ the set of time periods. $c^o_g$, $c^s_g$, $\underline{P}_g$, and $\overline{P}_g$ are respectively the production cost, startup cost, and the lower and upper production limits of generator $g\in\mc{G}$. For generator $g\in\mc{G}$ at time $t\in\mc{T}$, $p_{gt}$ is the production level, $u_{gt}$ is the binary decision to startup, and $z_{gt}$ is equal to one if online and zero if offline.
%Let $g\in\mc{G}$ be the index for generators in set $\mc{G}$, $t\in\mc{T}$ be the index for time in time period $\mc{T}$, $c^o_g$ and $c^s_g$ are respectively the costs of production and start up for generator $g$, $\underline{P}_g$ and $\overline{P}_g$ are respectively the lower and upper bounds for production levels of generator $g$. Additionally, we have three decision variables: for generator $g$ at hour $t$, $p_{gt}$ represents the production level, $u_{gt}$ is a binary variable that equals 1 if the generator is started up (0 otherwise), and $z_{gt}$ is a binary variable that equals 1 if the generator is on (0 otherwise). 
We deal with the following UC problem with load constraints and production level constraints \citep{carrion2006computationally, taylor2015convex}:%\footnotemark
%\footnotetext{\cred We can also incorporate additional constraints, such as minimum up/down time, ramping constraints, and energy storage, without no conceptual change. We omit these constraints for concision.}
%\begin{subequations}\label{eq: uc1}
%\begin{alignat}{4}
%\quad\min \quad& \sum_{g\in\mc{G}}\sum_{t\in\mc{T}} \Big(c^o_g p_{gt} + c^s_g u_{gt}\Big)\\
%\st \quad& \sum_{g\in\mc{G}}p_{gt} = d_t && \forall t\in\mc{T} \\
%& u_{gt} \geq z_{gt} - z_{g, t-1} && \forall g\in\mc{G}, t\in\mc{T}\sm\{1\}\\
%& p_{gt} \geq z_{gt} \underline{P}_g && \forall g\in\mc{G}, t\in\mc{T}\\
%& p_{gt} \leq z_{gt} \overline{P}_g && \forall g\in\mc{G}, t\in\mc{T}\\
%&u_{gt}, z_{gt}\in\{0,1\} \quad&~~& \forall g\in\mc{G},t\in\mc{T}\\
%&p_{gt} \geq 0 \quad&~~& \forall g\in\mc{G},t\in\mc{T}
%\end{alignat}
%\end{subequations}
\begin{subequations}\label{eq: uc1_reform}
\begin{alignat}{4}
\uc : \quad\min \quad& \sum_{g\in\mc{G}}\sum_{t\in\mc{T}} \Big(c^o_g p_{gt} + c^s_g u_{gt}\Big)\label{eq: uc1_reform_1}\\
\st \quad& \sum_{g\in\mc{G}}p_{gt} = d_t && \forall t\in\mc{T}\label{eq: uc1_reform_2} \\
& u_{gt} -\ddot{\theta}_{gt} = z_{gt} - z_{g, t-1} && \forall g\in\mc{G}, t\in\mc{T}\sm\{1\}\label{eq: uc1_reform_3}\\
& p_{gt} - \ddot{\mu}_{gt}= z_{gt} \underline{P}_g && \forall g\in\mc{G}, t\in\mc{T}\label{eq: uc1_reform_4}\\
& p_{gt} + \ddot{\gamma}_{gt} = z_{gt} \overline{P}_g && \forall g\in\mc{G}, t\in\mc{T}\label{eq: uc1_reform_5}\\
& u_{gt} + \ddot{\eta}_{gt} = 1 && \forall g\in\mc{G}, t\in\mc{T} \label{eq: uc1_reform_6}\\
%&z_{gt} + \ddot{\eta}_{gt} = 1 &&\forall g\in\mc{G}, t\in\mc{T}&&&{(\eta_{gt})}\label{eq: uc1_reform_6}\\
& z_{gt} \in\{0,1\}&&\forall g\in\mc{G}, t\in\mc{T}\\
&p_{gt},u_{gt}, \ddot{\theta}_{gt}, \ddot{\mu}_{gt}, \ddot{\gamma}_{gt}, \ddot{\eta}_{gt} \geq 0 \quad&~~& \forall g\in\mc{G},t\in\mc{T}.%, \ddot{\eta}_{gt}
\end{alignat}
\end{subequations}

$\ddot{\theta}_{gt}, \ddot{\mu}_{gt}, \ddot{\gamma}_{gt}$, and $\ddot{\eta}_{gt}$ are slack variables. The objective \eqref{eq: uc1_reform_1} is the total production and start up cost. Constraints \eqref{eq: uc1_reform_2} ensure that the total production satisfies the load at each hour. Constraint \eqref{eq: uc1_reform_3} relates variables $u_{gt}$ and $z_{gt}$. Constraint \eqref{eq: uc1_reform_4} and \eqref{eq: uc1_reform_5} limit the production levels. The integrality of $u_{gt}$ is implied by \eqref{eq: uc1_reform_3}.

%{\cred Note that for the convenience of CPP reformulation, which only works with models containing equality constraints, we add slack variables for all inequality constraints, including variables $\ddot{\theta}_{gt}, \ddot{\mu}_{gt}, \ddot{\gamma}_{gt}$, and $\ddot{\eta}_{gt}$. The objective function \eqref{eq: uc1_reform_1} minimizes the total production and start up costs. Constraints \eqref{eq: uc1_reform_2} ensure that total production satisfy load at each hour. Constraints \eqref{eq: uc1_reform_3} connects variables $u_{gt}$ and $z_{gt}$. Constraint \eqref{eq: uc1_reform_4} and \eqref{eq: uc1_reform_5} give the lower and upper bounds for production levels. We relax the $u_{gt}$ as a continuous variable, as its integrality is implied by constraints \eqref{eq: uc1_reform_3}. }

Note that we could in principle incorporate a number of additional constraints, such as minimum up/down time, ramping constraints, and energy storage, without no conceptual change. We omit these constraints for concision.

%---------%
\subsection{CPP Reformulation of UC}\label{subch: uc_reform}
%For the convenience of CPP reformulation, which only works with models containing equality constraints, we rewrite problem \eqref{eq: uc1} to add slack variables for all inequality constraints:
%Notice that in the reformulation above, we eliminate the binary constraints on $u_{gt}$. This is valid because in the minimization problem $~\uc$, constraints \eqref{eq: uc1_reform_3} and $u_{gt}\geq 0$ ensure that $u_{gt}$ is either 0 or 1. %We also add constraints \eqref{eq: uc1_reform_6} for , replacing them with constraint \eqref{eq: uc1_reform_6} and \eqref{eq: uc1_reform_7}. 
%%----%
%\subsection{CPP Reformulation}

We reformulate \eqref{eq: uc1_reform} in the form of $\mc{P}^{\text{CPP}}_o$. Let
 \[{\bf x}^\top = ({\mathbf u^\top}, {\mathbf z}^\top, {\mathbf p}^\top, \ddot{\pmb \theta}^\top, \ddot{\pmb \mu}^\top, \ddot{\pmb \gamma}^\top, \ddot{\pmb \eta}^\top) \] %, \ddot{\eta}_{[gt]}
where ${\mathbf u}$ is the vector of variables $u_{gt}$ for all $g\in\mc{G}, t\in\mc{T}$. Let $X$ be the matrix of lifted variables for $\x$. $Y$ is as defined in \eqref{eq: define_vars}. To make the correspondence between elements of $X$ and variables in vector $\x$ more explicit, we denote $X_{ii}$, the diagonal terms of $X$, as $V_k$, where $V$ is the upper case of $i^{\textrm{th}}$ variable and $k$ is its index. For example, $X_{22}$ is denoted as $U_{12}$, as the second variable in $x$ is $u_{12}$. Similarly, denote off-diagonal terms in $X$ as $X_{ij} = [V^1 V^2]_{k_1, k_2} (\forall i\neq j, i,j = 1,...,n$), where $V^1$ is the upper case of the $i^{\textrm{th}}$ variable in $x$ and $k_1$ is its index. So $X_{12} = [UU]_{11,12}$. Also, for the convenience of writing lifted constraints, we use vectors $\alambda$, $\a^{\theta_{gt}}$, $\a^{\mu_{gt}}$ $\a^{\gamma_{gt}}$, and $\aeta$ to respectively represent the parameter vectors of constraints \eqref{eq: uc1_reform_2} - \eqref{eq: uc1_reform_6}. The CPP reformulation is as follows\footnotemark: %Also, assume problem \eqref{eq: uc1_reform} satisfies Assumption \eqref{a: alpha}.
\begin{subequations}\label{eq: uc1_cpp1}
\begin{alignat}{4}
\uc^\cpp : \min \quad& \sum_{g\in\mc{G}}\sum_{t\in\mc{T}} \Big(c^o_g p_{gt} + c^s_g u_{gt}\Big)\hspace{1cm}\label{eq: uc1_cpp1_0}\\
\st \quad& \sum_{g\in\mc{G}}p_{gt} = d_t && \forall t\in\mc{T} &&&(\lambda_t)\label{eq: uc1_cpp1_1}\\
& u_{gt} -\ddot{\theta}_{gt} = z_{gt} - z_{g, t-1} && \forall g\in\mc{G}, t\in\mc{T}\sm\{1\}\hspace{1cm}&&&(\theta_{gt})\label{eq: uc1_cpp1_2}\\
& p_{gt} - \ddot{\mu}_{gt}= z_{gt} \underline{P}_g && \forall g\in\mc{G}, t\in\mc{T}&&&(\mu_{gt})\label{eq: uc1_cpp1_lim1}\\
& p_{gt} + \ddot{\gamma}_{gt} = z_{gt} \overline{P}_g && \forall g\in\mc{G}, t\in\mc{T}&&&(\gamma_{gt})\label{eq: uc1_cpp1_lim2}\\
&u_{gt} + \ddot{\eta}_{gt} = 1 &&\forall g\in\mc{G}, t\in\mc{T}&&&{(\eta_{gt})} \label{eq: uc1_cpp1_ub}\\
&\tr(\alambda \alambdatop X) = d_t^2&&\forall t\in\mc{T}&&&(\Lambda_t)\label{eq: uc1_cpp1_7}\\
&\tr(\a^{\theta_{gt}} \athetatop X) = 0&&\forall g\in\mc{G}, t\in\mc{T}\sm\{1\}&&&(\Theta_{gt})\label{eq: uc1_cpp1_8}\\
&\tr(\a^{\mu_{gt}} \a^{\mu_{gt} \top} X) = 0&&\forall g\in\mc{G},t\in\mc{T}&&&(M_{gt})\\
&\tr(\a^{\gamma_{gt}} \a^{\gamma_{gt} \top} X) = 0&&\forall g\in\mc{G},t\in\mc{T}&&&(\Gamma_{gt})\label{eq: uc1_cpp1_10}\\
&\tr(\aeta \aetatop X) = 1&&\forall g\in\mc{G},t\in\mc{T}&&&(H_{gt})\label{eq: uc1_cpp1_11}\\
%&u_{gt} = U_{gt} &&\forall g\in\mc{G},t\in\mc{T}&&&(\delta^{(1)}_{gt})\\
&z_{gt} = Z_{gt} &&\forall g\in\mc{G},t\in\mc{T}&&&(\delta_{gt})\label{eq: uc1_cpp1_13}\\
&Y\in\mc{C}_{n+1}^*&& &&&(\Omega).\label{eq: uc1_cpp1_14}
\end{alignat}
\end{subequations}
%\footnotetext{\cred We use lower and upper case Greek letters to denote the dual variables for original constraints and their corresponding lifted constraints.}

Dual variables are shown to the right of the constraints. %{\cred For simplicity, we write the left-hand sides of lifted constraints \eqref{eq: uc1_cpp1_7} - \eqref{eq: uc1_cpp1_11} in the trace form. For example, the explicit form of $\tr(\aeta \aetatop X)$ is $Z_{gt}^* +  \ddot{H}^*_{gt} + 2 [Z\ddot{H}]^*_{gt,t}$.}

The dual of \eqref{eq: uc1_cpp1} is:
\begin{subequations}\label{eq: uc1_cop}
\begin{alignat}{4}
\uc^\cop: \max~~&\sum_{t\in\mc{T}}\Big(\lambda_t d_t + \Lambda_t d_t^2 + \sum_{g\in\mc{G}}\left(\eta_{gt} + H_{gt}\right)\Big)\label{eq: uc1_cop_obj}\\ %
\st ~~&(\pmb \lambda, \pmb \theta, \pmb \mu, \pmb \gamma, \pmb \eta, \pmb \Lambda, \pmb \Theta, {\mathbf M}, \pmb \Gamma, {\mathbf H}, \pmb \delta, \Omega)\in\mc{F}^{\text{COP}},\label{eq: uc1_cop_constr}
\end{alignat}
\end{subequations}
where $\mc{F}^{\text{COP}}$ denotes the feasible region of the dual problem characterized by constraints in the form of constraints \eqref{eq: cop_origin_2} - \eqref{eq: cop_origin_3}.
%Since CPP \eqref{eq: uc1_cpp1} is a convex program, if it satisfies certain sufficient conditions such as Slater's condition, then strong duality holds. This means at an optimum, the primal objective \eqref{eq: uc1_cpp1_0} is equivalent to the dual objective \eqref{eq: uc1_cop_obj}. 

% For the convenience of the discussion that follows, we assume whenever we mention an optimal solution of CPP \eqref{eq: uc1_cpp1}, i.e. $(\x^*, X^*)$, we assume its componet $\x^*$ solves the original MIP formulation \eqref{eq: uc1_reform}. This assumption is not restrictive, as such an $\x^*$ always exists according to Proposition \ref{th: qip_sol}.
%---------%
\subsection{Copositive Duality Pricing Mechanism}\label{subch: pricing_mechanism}
We now describe CDP, a pricing scheme for UC. CDP is budget balanced and, under certain conditions, individually rational.


use copositive duality to construct a pricing scheme for UC, we would like to find a market mechanism where the total payments are enough to cover the total costs. Strong duality of CPP enables us to derive such a market mechanism, where we use the dual variables that appear in the dual objective \eqref{eq: uc1_cop_obj} as prices. More specifically, let $\x^*$ be the optimal solution of the original UC MIP problem \eqref{eq: uc1_reform}, and $X^* = \x^* \x^{*\top}$. Then according to Remark \ref{th: qip_sol}, $(\x^*, X^*)$ is an optimal solution to $\uc^\cpp$ \eqref{eq: uc1_cpp1}. Let $(\pmb \lambda^*, \pmb \eta^*, \pmb \Lambda^*, {\mathbf H}^*)$ be a set of optimal dual solutions {\cred for $\uc^\cop$}.
%, and multiply the left-hand side of constraints \eqref{eq: uc1_cpp1_1}, \eqref{eq: uc1_cpp1_ub}, \eqref{eq: uc1_cpp1_7}, and \eqref{eq: uc1_cpp1_11} with corresponding dual prices  (substitute the primal variables with optimal values too). 
{\cred We call the set of dual prices $(\pmb \lambda^*, \pmb \eta^*, \pmb \Lambda^*, {\mathbf H}^*)$ the {\it CDP prices}. We propose a market mechanism based on the CDP prices where the total payment from the system operator to generators, $\pi^\so$, depends on generators' optimal production levels and on/off statuses. More specifically, $\pi^\so$ is the sum of products between the left-hand sides of constraints \eqref{eq: uc1_cpp1_1}, \eqref{eq: uc1_cpp1_ub}, \eqref{eq: uc1_cpp1_7}, and \eqref{eq: uc1_cpp1_11} with corresponding dual prices (We will explain the meanings of those products later). So $\pi^\so$ includes the products of $\lambda_{t}^*$ and $\sum_{g\in\mc{G}} p^*_{gt}$, $ \eta_{gt}^*$ and $z_{gt}^*+\ddot{\eta}^*_{gt}$, $\Lambda_{t}^*$ and $\tr(\alambda \alambdatop X) = \sum_{g\in\mc{G}} P_{gt}^* + 2\sum_{g_1< g_2, g_1,g_2 \in\mc{G}} [PP]^*_{g_1 t, g_2 t}$, and $H_{[gt]}^*$ and $\tr(\aeta \aetatop X) = Z_{gt}^* +  \ddot{H}^*_{gt} + 2 [Z\ddot{H}]^*_{gt,t}$. That is to say, $\pi^\so$ equals: }
%Denoting the total payments as $\pi^\so$, as this payment is obtained from solving the system operator's aggregated cost minimization problem, then $\pi^\so$ is calculated as follows:%, $\eta_{[gt]}^*$, $H_{[gt]}^* , \eqref{eq: uc1_cpp1_7}, and \eqref{eq: uc1_cpp1_11}
\begin{align}
&\sum_{t\in\mc{T}}\bigg(\sum_{g\in\mc{G}}\Big(\lambda_t^* p^*_{gt} + \eta^*_{gt} z^*_{gt} + \eta^*_{gt} \ddot{\eta}^*_{gt} + \Lambda^*_t P_{gt}^*\Big) + 2\sum_{g_1< g_2, g_1,g_2 \in\mc{G}}\Lambda^*_t [PP]^*_{g_1 t, g_2 t} \nonumber\\
&  + \sum_{g\in\mc{G}}\Big(H_{gt}^* Z_{gt}^* + H_{gt}^* \ddot{H}^*_{gt} + 2 H_{gt}^* [Z\ddot{H}]^*_{gt,t}\Big)\bigg).
\end{align}%
%where $ \sum_{g\in\mc{G}} \Lambda^*_t P_{gt}^* + 2\sum_{g_1< g_2, g_1,g_2 \in\mc{G}}\Lambda^*_t [PP]^*_{g_1 t, g_2 t}$ represents the explicit form of $\Lambda^*_t \tr(\alambda \alambdatop X)$, and $H_{gt}^* Z_{gt}^* + H_{gt}^* \ddot{H}_{gt} + 2 H_{gt}^* [Z\ddot{H}]^*_{gt,t}$ represents the explicit form of $H^*_{gt} \tr(\aeta \aetatop X)$. 

Because of \eqref{eq: uc1_cpp1_ub} and \eqref{eq: uc1_cpp1_11}, we can equivalently replace $\eta^*_{gt} z^*_{gt} + \eta^*_{gt} \ddot{\eta}^*_{gt}$ with $\eta^*_{gt}$ and replace $H_{gt}^* Z_{gt}^* + H_{gt}^* \ddot{H}_{gt} + 2 H_{gt}^* [Z\ddot{H}]^*_{gt,t}$ with $H^*_{gt}$, and rewrite $\pi^\so$ as follows:
\begin{align}
\pi^\so =  &\sum_{t\in\mc{T}}\bigg(\sum_{g\in\mc{G}}\Big(\lambda_t^* p^*_{gt} + \eta^*_{gt} + \Lambda^*_t P_{gt}^*\Big) + 2\sum_{g_1< g_2, g_1,g_2 \in\mc{G}}\Lambda^*_t [PP]^*_{g_1 t, g_2 t} + \sum_{g\in\mc{G}}H_{gt}^*\bigg).\label{eq:pisopayment}
\end{align}

The term $\lambda_t^* p^*_{gt}$ is the payment from the uniform production price $\lambda_t^*$, corresponding to the demand constraint \eqref{eq: uc1_cpp1_1}. Payment $\Lambda^*_t P_{gt}^*$ is also a payment from uniform price, $\Lambda^*_t$, which corresponds to the lifted demand constraint \eqref{eq: uc1_cpp1_7}. However, there is an extra payment from this lifted constraint, i.e. $\Lambda^*_t [PP]^*_{g_1 t, g_2 t}$, which depends on an off-diagonal term of $X^*$. Since this payment involves two generators, it is an open question as to how this payment should be divided between those generators. {\cred For example, we can assign it to the generator that loses money, or divide it evenly (this is the option we choose for the RCDP in Section \ref{subch: mod_cop_pricing}).} %One way to divide this payment is to approximately linearize $[PP]^*_{g_1 t, g_2 t}$. Because of Lemma \ref{th: qip_sol2}, at optimality of CPP, one of the optimal solutions should satisfy $X^* = \x^* \x^{*\top}$, with $\x^*$ being the optimal solution of $~\uc$. For this solution, $[PP]^*_{g_1 t, g_2 t} = p^*_{g_1 t} p^*_{g_2 t}$. If either one of $p^*_{g_1 t}$ and $p^*_{g_2 t}$ is 0, then the payment for the crossed term is 0. Otherwise, $\underline{P}_g \leq  p^*_{gt} \leq \bar{P_g}, g = g_1, g_2$. With those bounds, we obtain the following inequalities via the McCormick relaxation:
%\begin{subequations}\label{eq: mccormick}
%\begin{alignat}{4}
%p^*_{g_1 t} p^*_{g_2 t} &\geq {\underline P_{g_2}} p^*_{g_1 t} +{\underline P_{g_1}}  p^*_{g_2 t} - {\underline P_{g_1}}{\underline P_{g_2}}\\
%p^*_{g_1 t} p^*_{g_2 t} &\geq {\bar P_{g_2}} p^*_{g_1 t} +{\bar P_{g_1}}  p^*_{g_2 t} - {\bar P_{g_1}}{\bar P_{g_2}}\\
%p^*_{g_1 t} p^*_{g_2 t} &\leq {\underline P_{g_2}} p^*_{g_1 t} +{\bar P_{g_1}}  p^*_{g_2 t} - {\bar P_{g_1}}{\underline P_{g_2}}\\
%p^*_{g_1 t} p^*_{g_2 t}& \leq {\bar P_{g_2}} p^*_{g_1 t} +{\underline P_{g_1}}  p^*_{g_2 t} - {\underline P_{g_1}}{\bar P_{g_2}}
%\end{alignat}
%\end{subequations}
%Sum up the right-hand sides of inequalities in \eqref{eq: mccormick}, divide by 4, and rearrange, we get an approximation for the bilinear term $p^*_{g_1 t} p^*_{g_2 t}$: $0.5 ({\underline P_{g_2}} + {\bar P_{g_2}}) (p^*_{g_1 t} - 0.5 \underline{P_{g_1}}) +0.5({\underline P_{g_1}}+ {\bar P_{g_1}}) (p^*_{g_2 t} - 0.5 \underline{P_{g_2}})$. Therefore, the payment $2 \Lambda^*_t [PP]^*_{g_1 t, g_2 t}$ can be divided by paying generator $g_1$ at unit price $ \Lambda^*_t({\underline P_{g_2}}+{\bar P_{g_2}})$ for the production that is above $0.5{\underline P_{g_1}}$. $g_2$ is paid similarly. 
Payments $\eta^*_{gt}$ and $H_{gt}^*$ are the generator-dependent payments corresponding to constraints \eqref{eq: uc1_cpp1_ub} and \eqref{eq: uc1_cpp1_11}, respectively. Since the prices $\eta^*_{gt}$ and $H_{gt}^*$ signals the availability of generators at each hour, we name them the {\it availability prices}. 
%Finally, we use the name {\it CDP prices} for the prices $(\pmb \lambda^*, \pmb \eta^*, \pmb \Lambda^*, {\mathbf H}^*)$ that consist the total payment $\pi^\so$.

%----%
\subsubsection{Revenue Neutrality}
%It can be proved that the market mechanism with the total payment $\pi^\so$ equals the total cost, i.e., is revenue neutral {\cred (We include the proof of Theorem \ref{th: rev_adequacy} in the text as some of its deduction steps will be useful later.)}: %It can be proved that t via the strong duality of CPP 
We now prove that CDP is revenue neutral.

% === Theorem ====
\begin{theorem}\label{th: rev_adequacy}
%Assume the CPP reformulation of $~\uc$, i.e. \eqref{eq: uc1_cpp1}, satisfies some regularity condition for convex programming strong duality. Then CDP is revenue neutral.
If strong duality holds for $\uc^\cpp$, then CDP is revenue neutral.
\end{theorem}

\proof{Proof.}
Fix all primal and dual variables at the optimal values, and multiply the following constraints by their corresponding dual variables: \eqref{eq: uc1_cpp1_2}, \eqref{eq: uc1_cpp1_ub}, \eqref{eq: uc1_cpp1_7}, and \eqref{eq: uc1_cpp1_11}. This gives 
\begin{subequations}\label{eq: uc1_balance}
\begin{alignat}{4}
& \sum_{g\in\mc{G}}\lambda_t^* p^*_{gt} = \lambda_t^* d_t && \forall t\in\mc{T} \label{eq: uc1_balance_1}\\
&\eta^*_{gt} z^*_{gt} + \eta^*_{gt} \ddot{\eta}^*_{gt} = \eta^*_{gt} &&\forall g\in\mc{G}, t\in\mc{T} \label{eq: uc1_balance_ub}\\
&\sum_{g\in\mc{G}} \Lambda^*_t P_{gt}^* + 2\sum_{g_1< g_2, g_1,g_2 \in\mc{G}}\Lambda^*_t [PP]^*_{g_1 t, g_2 t} = \Lambda^*_t d_t^2&~~~&\forall t\in\mc{T}\\
& H_{gt}^* Z_{gt}^* + H_{gt}^* \ddot{H}_{gt} + 2 H_{gt}^* [Z\ddot{H}]^*_{gt,t} = H_{gt}^*  &~&\forall g\in\mc{G}, t\in\mc{T}.
\end{alignat}
\end{subequations}
Sum the equations in \eqref{eq: uc1_balance} over their indices, and then sum the results. The left-hand side represents the total payments, $\pi^\so$, and the right-hand side is the optimal value of the dual objective \eqref{eq: uc1_cop_obj}:
\begin{align}\label{eq: payment_dual_obj}
\pi^\so = \sum_{t\in\mc{T}}\Big(\lambda^*_t d_t + \Lambda^*_t d_t^2 + \sum_{g\in\mc{G}}(\eta^*_{gt} + H^*_{gt})\Big).
\end{align}

Because we have assumed that strong duality holds for $\uc^\cpp$, the right-hand side of \eqref{eq: payment_dual_obj} equals the optimal objective of the primal problem. Thus,
\[
\pi^\so = \sum_{g\in\mc{G}}\sum_{t\in\mc{T}} \Big(c^o_g p^*_{gt} + c^s_g u^*_{gt}\Big).
\]
Therefore, the total payment from the load equals the total cost.
\Halmos\endproof
% === End of Theorem ====
This result shows that the system operator is budget balanced, i.e., the payment it receives from the loads is equal to its payments to the generators. It also shows that the total payment to the generators is equal to the total cost of the generators.

%Equation \eqref{eq: payment_dual_obj} indicates that the utility's revenue and costs are balanced under CDP, as the left-hand side of \eqref{eq: payment_dual_obj} is utility's total payments to generators, and the right-hand side of  \eqref{eq: payment_dual_obj} represents utility's total revenue from consumers.
%----%
\subsubsection{Individual Rationality}\label{subch: individual_rational}
A pricing mechanism is individually rational if each market participant has no incentive to deviate from the centrally optimal solution. We now analyze when CDP is individually rational.

The profit-maximization problem of generator $g$ is given by:
\begin{subequations}\label{eq: uc1_individual}
\begin{alignat}{4}
\pi_g^\gen (\p_{-g}) := \quad\max_{\xg} \quad& \sum_{t\in\mc{T}} \Big(\lambda^*_t p_{gt} + \eta^*_{gt} + \Lambda^*_t p_{gt}^{2} + H^*_{gt} +\sum_{g'\in -g}f(p_{gt}, p_{g't})\nonumber\hspace{-3cm}\\&- c^o_g p_{gt} - c^s_g u_{gt}\Big)\label{eq: uc1_individual_1}\\
\st \quad& u_{gt} -\ddot{\theta}_{gt} = z_{gt} - z_{g, t-1} && \forall t\in\mc{T}\sm\{1\}&&~~&\label{eq: uc1_individual_2}\\
& p_{gt} - \ddot{\mu}_{gt}= z_{gt} \underline{P}_g && \forall t\in\mc{T}\\
& p_{gt} + \ddot{\gamma}_{gt} = z_{gt} \overline{P}_g &&\forall t\in\mc{T}\\
%&z_{gt} + \ddot{\eta}_{gt} = 1 &&\forall  t\in\mc{T}&&&{(\eta_{gt})}\\
& u_{gt}, z_{gt}\in\{0,1\} &~~&\forall t\in\mc{T}\\
&p_{gt}, \ddot{\theta}_{gt}, \ddot{\mu}_{gt}, \ddot{\gamma}_{gt}\geq 0 \quad&~~& \forall t\in\mc{T}, \label{eq: uc1_individual_6}
\end{alignat}
\end{subequations}
where $-g = \mc{G}\sm g$ and $\p_{-g}$ denotes the production decision of all generators other than $g$. $\xg\in\mb{R}^{n_g}$ denotes the portions of $\x$ that corresponds to generator $g\in\mc{G}$. The first five terms in the objective represent the total revenue of generator $g$. $f(p_{gt}, p_{g't})$ is the share of $g$'s revenue from the cross-term payment $2\Lambda_t^* [PP]_{g t, g' t}$, and $f(p_{gt}, p_{g't}) + f(p_{g't}, p_{gt}) = 2\Lambda_t^* p_{g} p_{g'}$. Also, if $p_{g} p_{g'} = 0$ then $f(p_{gt}, p_{g't}) = 0$. Notice that $\pi_g^\gen (\p_{-g})$ should not contain $X$. This is why we need to rewrite the cross-term payment in terms of $p_{gt}$'s. We assume that at optimality $P^*_{gt} = (p^{*}_{gt})^2$ and $[PP]^*_{g t, g' t} = p^*_{gt} p^*_{g' t}$. This replacement is valid because of Remark \ref{th: qip_sol}.
%Notice that in order to formulate the individual generator's profit-maximization problem, which does not have variables from $X$, we need to assume that at optimality $P^*_{gt} = (p^{*}_{gt})^2$ and $[PP]^*_{g t, g' t} = p^*_{gt} p^*_{g' t}$ for $\uc^\cpp$, so replacing lifted terms with polynomials of $p_{[gt]}$ for revenue is valid. This replacement is valid because of Remark \ref{th: qip_sol}.

If the optimal solution of the profit-maximization problem \eqref{eq: uc1_individual} matches the corresponding portion of the optimal solution of $~\uc$ for all generators $g\in\mc{G}$, then the market mechanism is individually rational.

Theorem \ref{th: ind_rational} provides a sufficient condition for when CDP is individually rational. We first need the following lemma. %But before proving Theorem \ref{th: ind_rational} we need the following lemma, which shows that constraint $Y\in\mc{C}_{n+1}^*$ is decomposable by generators under certain conditions: {\cgreen (Cheng: could move to appendix if more space is needed)}
% === Lemma ====
\begin{lemma}\label{th: separate_conic}
Let $\xg\in\mb{R}^{n_g}$ and $X_g\in\mb{R}^{n_g \times n_g}$ denote the portions of $\x$ and $X$ that correspond to generator $g\in\mc{G}$, and let 
$Y_g = \left[\begin{array}{cc}
1 & {\bf x}_g^\top \\
{\bf x}_g & X_g
\end{array}\right].$
If all terms in $X$ of the form $[V^1 V^2]_{g_1 t, g_2 t}, \forall g_1 \neq g_2, g_1,g_2\in\mc{G}, t\in\mc{T}$ are equal to zero, then the conic constraint $Y\in\mc{C}_{n+1}^*$ is equivalent to constraints \eqref{eq: uc1_individual_conic}:
\begin{align}\label{eq: uc1_individual_conic}
Y_g \in\mc{C}_{n_g + 1}^* ~~\forall g\in\mc{G},
\end{align}
which ensure that $Y_g$ is copositive for all $g\in\mc{G}$.
%Now we introduce constraints \eqref{eq: uc1_individual_conic}:
%\begin{subequations}\label{eq: uc1_individual_conic}
%\begin{alignat}{4}
%&Y^g \in\mc{C}^*&&\forall g\in\mc{G}\label{eq: uc1_individual_conic_1}\\
%&[V^1 V^2]^*_{g_1 t, g_2 t} = 0 &~~& \forall g_1 \neq g_2, g_1,g_2\in\mc{G}, t\in\mc{T}\label{eq: uc1_individual_conic_2}
%\end{alignat}
%\end{subequations}
%where constraints \eqref{eq: uc1_individual_conic_1} ensure that $Y^g$ is copositive for all $g\in\mc{G}$. Constraints \eqref{eq: uc1_individual_conic_2} ensure that all off-diagonal terms of $X$ that correspond to two different generators should equal to zero.
%Then constraints \eqref{eq: uc1_individual_conic} hold if and only if constraints \eqref{eq: fix_cross_gen_X} are satisfied:
%\begin{subequations}\label{eq: fix_cross_gen_X}
%\begin{alignat}{4}
%&Y\in\mc{C}^*\\
%&[V^1 V^2]^*_{g_1 t, g_2 t} = 0 &~~&\forall g_1 \neq g_2, g_1,g_2\in\mc{G}, t\in\mc{T}\label{eq: fix_cross_gen_X_2}
\end{lemma}
% === End of Lemma ====
Now we are ready to prove Theorem \ref{th: ind_rational}:
% === Theorem ====
\begin{theorem}\label{th: ind_rational}
Assume CPP \eqref{eq: uc1_cpp1} satisfies some sufficient condition for convex programming strong duality. Additionally, let $(\x^*, X^*)$ be an optimal solution for the problem \eqref{eq: uc1_cpp1}, if all items in $X^*$ in the forms of $[V^1 V^2]^*_{g_1 t, g_2 t}, \forall g_1 \neq g_2, g_1,g_2\in\mc{G}, t\in\mc{T}$ are equal to zero, then the market mechanism with CDP is individually rational.
\end{theorem}
% === End of Theorem ====

It is straightforward to see that if there is only one generator in the system, our market mechanism is individually rational, because there will be no crossed terms in the form of $[V^1 V^2]_{g_1 t, g_2 t}$ in the problem. %the payment $\pi^\so$ induced by $[\lambda^*_t, \eta^*_{gt}, \Lambda^*_t, H^*_{gt}]$

We can extend the concept of individual rationality of a single generator to the behaviour of a subset of generators that are owned by the same company. Let generators in $\mc{G}$ be grouped into $n$ disjoint subsets $\mc{G}_{1}, ...,\mc{G}_{n}$, and each subset of generators jointly solve their own profit-maximization problem. We call a market mechanism {\it subset rational} if given the prices, each subset of generators do not have the incentive to deviate from the designated production level. We omit the discussion for the sufficient condition because it is similar to above.

\begin{comment}
{\cgreen (Cheng: Merve, I still think it's better to start a new paragraph here)}We can extend the concept of individual rationality of a single generator to the behaviour of a subset of generators that are owned by one company. Let generators in $\mc{G}$ be grouped into $n$ disjoint subsets $\mc{G}_{1}, ...,\mc{G}_{n}$, and each subset of generators jointly solve their own profit-maximization problem. We call a market mechanism {\it subset rational} if given the prices, each subset of generators do not have the incentive to deviate from the designated production level. The profit-maximization problem solved by generators in the subset $\mc{G}_i, i\in\{1,...,n\}$ is as follows:
\begin{subequations}\label{eq: uc1_subset}
\begin{alignat}{4}
\pi_{\mc{G}_i}(\p_{- \mc{G}_i}): \max \quad& \sum_{t\in\mc{T}} \Bigg(\sum_{g\in\mc{G}_i}\Big(\lambda^*_t p_{gt}+\eta_{gt}^* + \Lambda^*_t (p_{gt})^2 + H_{gt}^* +\sum_{g'\in\mc{G}\sm\mc{G}_i}f(p_{gt}, p_{g't})\hspace{-3cm}\nonumber\\ & - c^o_g p_{gt} - c^s_g u_{gt}\Big) + \sum_{g<g', g, g'\in\mc{G}_i}2 \Lambda^*_t p^*_{gt} p^*_{g't} \Bigg)&&\\
\st \quad&\eqref{eq: uc1_individual_2} - \eqref{eq: uc1_individual_6} &&\forall g\in\mc{G}_i.
\end{alignat}
\end{subequations}

Corollary \ref{th: group_rational} provides a sufficient condition for subset rationality, which is less restrictive than the sufficient condition for individual rationality in Theorem \ref{th: ind_rational}:
% === Corollary ====
\begin{corollary}\label{th: group_rational}
Assume CPP \eqref{eq: uc1_cpp1} satisfies some sufficient condition for convex programming strong duality. Additionally, let $(\x^*, X^*)$ be an optimal solution for the problem \eqref{eq: uc1_cpp1}, if all items in $X^*$ in the forms of $[V^1 V^2]^*_{g_1 t, g_2 t}, \forall g_1 \in\mc{G}_i, g_2\in\mc{G}_j, i\neq j, i,j = 1,...,n; t\in\mc{T}$ are equal to zero, then the market mechanism with total payment $\pi^\so$ is also subset rational.
\end{corollary}
The proof of Corollary \ref{th: group_rational} follows similar steps as the proof of Theorem \ref{th: ind_rational}, so we do not repeat it.
% === End of Corollary ====
\end{comment}
% Another perspective for individual rationality is to view the market as a game induced by the pricing mechanism $\pi^\so$, with the generators as players. In such a game, each generator $g$ solves the profit-maximizing problem \eqref{eq: uc1_individual}, while treating $\x_{-g}$, the decisions from other generators, as given. A solution $\x^*$ constitutes a Nash equilibrium if $\pi_g^\gen(\xstarg, \x_{-g}^*) \geq \pi_g^\gen(\xg, \x_{-g}^*)$, where $\xg$ represents any feasible strategies for $g$. Then a market mechanism is individually rational if the Nash equilibrium solution $\x^*$ is also optimal for the utility's problem $~\uc$. 
%
%The game induced by the pricing mechanism $\pi^\so$ is a mixed-binary quadratic game, which we will define in Section \ref{ch: app_game}. With COP duality, we are able to obtain theoretical results for the existence and uniqueness of Nash equilibria in mixed-integer quadratic games.

%-------------%
\subsection{Ensuring Individual Revenue Adequacy}\label{subch: mod_cop_pricing}
CDP does not guarantee each generator's revenue adequacy, i.e., nonnegative profit. This is also the case with some other schemes, including RP and CHP. In CDP, we can enforce revenue adequacy by adding constraints directly to the dual of $\uc^\cpp$.

There are two options for enforcing revenue adequacy: either through the uniform prices $\lambda_t$ and $\Lambda_t$, or through both the uniform prices and availability prices (which can be different for each generator).
%Revenue adequacy can be enforced through the availability prices, which can be different for each generator, or through the uniform prices $\lambda_t$ and $\Lambda_t$. 
We use the former, as uniform pricing is easier to implement in practice. In Section \ref{ec: ind_rev_avail_price} of the e-companion, we present a different version that uses availability prices as well.

%{ces as w\cred prell.iWe choose to develop a pricing scheme relying soley one uniform prices in this section, as this option is preferable in practice. For completeness, we include a pricing scheme with both revenue adequacy constraints and availability prices in e-companion Section \ref{ec: ind_rev_avail_price}.}

We enforce revenue adequacy by adding a new constraint to the dual problem, which ensures that the payment to each generator is no less than its costs. The resulting augmented dual problem is given by:
 %More specifically, for each generator $g$ define its share from the cross-term payment with generator $g'$ as $\pi^{\cross}_{gg'}$, and the total uplift payment for generator $g$ at hour $t$ as $\pi^{\uplift}_{g}$, we solve the following modified CDP problem
\begin{subequations}\label{eq: uc1_cop_profitable}
\begin{alignat}{4}
\max~~&\sum_{t\in\mc{T}}\Big(\lambda_t d_t + \Lambda_t d_t^2+ \sum_{g\in\mc{G}}(\eta_{gt} + H_{gt})\Big)\label{eq: uc1_cop_profitable_obj}\\ %+ \sum_{g\in\mc{G}}(\eta_{gt} + H_{gt}
\st ~~&\sum_{t\in\mc{T}} \Big(p^*_{gt}\lambda_t + p^{*2}_{gt} \Lambda_t + \sum_{g'\in\mc{G}\sm\{g\}} p_{gt}^*p_{g't}^*\Lambda_t \Big) \geq \sum_{t\in\mc{T}}\Big(c^o_g p^*_{gt} + c^s_g u^*_{gt}\Big) &~~~&\forall g\in\mc{G} \label{eq: uc1_cop_profitable_1}\\%+ \pi^\uplift_{g} + \eta_{gt} + H_{gt}
%&\pi^\extra_{g} + \sum_{g'\in\mc{G}\sm{\{g\}}}\pi^\cross_{gg'} = \pi^\uplift_{g} \label{eq: uc1_cop_profitable_2}\\
%&  \pi^\cross_{gg'} + \pi^\cross_{g'g} = \sum_{t\in\mc{T}} 2 p^*_{gt} p^*_{g't} \Lambda_t &&\forall g\neq g' \in\mc{G}  \label{eq: uc1_cop_profitable_3}\\
%& \pi^\extra_{g} \geq 0 &&\forall g\in\mc{G}\\
&(\pmb \lambda, \pmb \theta, \pmb \mu, \pmb \gamma, \pmb \eta, \pmb \Lambda, \pmb \Theta, {\mathbf M}, \pmb \Gamma, {\mathbf H}, \pmb \delta, \Omega)\in\mc{F}^{\text{COP}}.\hspace{-1cm}&&\label{eq: uc1_cop_profitable_constr}
\end{alignat}
\end{subequations}
The objective \eqref{eq: uc1_cop_profitable_obj} and the constraint \eqref{eq: uc1_cop_profitable_constr} are the same as in the original dual problem \eqref{eq: uc1_cop}. The left-hand side of constraint \eqref{eq: uc1_cop_profitable_1} is the total revenue of generator $g$, assuming that the cross-term payments are divided evenly between generators. The right-hand side of \eqref{eq: uc1_cop_profitable_1} is the total cost of generator $g$.

The prices are computed by solving \eqref{eq: uc1_cop_profitable}. The optimal values of primal variables, $p_{gt}^*$ and $u_{gt}^*$, could be obtained by solving $\uc$. We refer to this pricing mechanism as Revenue-adequate CDP (RCDP).

%Constraints \eqref{eq: uc1_cop_profitable_2} require that the total revenue from $g$'s share of cross-term payments equals the uplift. Constraints \eqref{eq: uc1_cop_profitable_3} define how cross-term payments are shared between generators.

A benefit of RCDP is that all generators are paid the same price in each hour, so that more efficient generators with lower costs earn higher profit. The load also no longer need to pay a fixed price. Generators getting paid by a uniform price also means that the total payments to generators might exceed their total costs. The system operator, however, remains budget balanced, in that the payment from the load at time $t$, $\lambda_t d_t + \Lambda_t d_t^2$, is always equal to the payment to the generators, 
$\sum_{g\in\mc{G}}\Big(p^*_{gt}\lambda_t + p^{*2}_{gt} \Lambda_t + \sum_{g'\in\mc{G}\sm\{g\}} p_{gt}^*p_{g't}^*\Lambda_t\Big)$. We can see this by equating \eqref{eq:pisopayment} and \eqref{eq: payment_dual_obj} and deleting the terms $\eta_{gt}$ and $H_{gt}$ from both sides.

%since we use only the uniform prices and ignore the availability prices $\eta_{gt}$ and $H_{gt}$, the total payments under RCDP no longer equals the total costs. However, the RCDP still balances the utility's revenue and payments. More specifically, the utility's revenue from demand at hour $t$ is $\lambda_t d_t + \Lambda_t d_t^2$, while its total payments to generators at hour $t$ is $\sum_{g\in\mc{G}}\Big(p^*_{gt}\lambda_t + p^{*2}_{gt} \Lambda_t + \sum_{g'\in\mc{G}\sm\{g\}} p_{gt}^*p_{g't}^*\Lambda_t\Big)$. We can prove that those two expressions are equivalent, by deleting eliminating terms of availability prices from both sides of \eqref{eq: payment_dual_obj}.
%According to equation \eqref{eq: payment_dual_obj} in the proof of Theorem \ref{th: rev_adequacy}, we have 
%\begin{align}\label{eq: modified_balance}
%&\sum_{t\in\mc{T}}\bigg(\sum_{g\in\mc{G}}\Big(\lambda_t^* p^*_{gt} + \eta^*_{gt} + \Lambda^*_t p_{gt}^{*2}\Big) + 2\sum_{g_1< g_2, g_1,g_2 \in\mc{G}}\Lambda^*_t p^*_{g_1 t}p^*_{g_2 t}+ \sum_{g\in\mc{G}}H_{gt}^*\bigg) \nonumber\\
%&= \sum_{t\in\mc{T}}\Big(\lambda^*_t d_t + \Lambda^*_t d_t^2 + \sum_{g\in\mc{G}}(\eta^*_{gt} + H^*_{gt})\Big)
%\end{align}
%eliminating terms of availability prices from both sides, we obtain the result we want, i.e. utility's total payments equals the revenue. 
%We formalize this result in the following theorem:
%\begin{proposition}
%The RCDP balances the utility's %revenue and payments.
%\end{proposition}

Because the addition of constraints \eqref{eq: uc1_cop_profitable_1} restrict the original dual problem \eqref{eq: uc1_cop}, it is worth checking if the problem is still feasible. We known that if either the primal or dual is feasible, bounded, and has an interior point, then the other is also feasible \citep{luenberger2015linear}. We therefore focus on the dual of \eqref{eq: uc1_cop_profitable}. Let $q_g \geq 0$ be the dual multiplier of \eqref{eq: uc1_cop_profitable_1}. The dual of \eqref{eq: uc1_cop_profitable} is the following:
\begin{subequations}\label{eq: uc1_cpp_profitable}
\begin{alignat}{4}
\min \quad& \sum_{g\in\mc{G}}\sum_{t\in\mc{T}} \Big(c^o_g p_{gt} + c^s_g u_{gt}- (c^o_g p^*_{gt} + c^s_g u^*_{gt})q_g\Big)\label{eq: uc1_cpp_profitable_0}\\
\st \quad& \sum_{g\in\mc{G}}\left(p_{gt} - p^*_{gt}q_g\right) = d_t && \forall t\in\mc{T} \label{eq: uc1_cpp_profitable_1}\\
&\tr(\alambda \alambdatop X) - \sum_{g\in\mc{G}} \Big(p^{*2}_{gt} + \sum_{g'\in\mc{G}\sm\{g\}} p_{gt}^*p_{g't}^*\Big)q_g= d_t^2&~~~&\forall t\in\mc{T}\label{eq: uc1_cpp_profitable_2}\\
& \eqref{eq: uc1_cpp1_2} - \eqref{eq: uc1_cpp1_ub}, \eqref{eq: uc1_cpp1_8}-\eqref{eq: uc1_cpp1_13}\\
&q_{g} \geq 0 &&g\in\mc{G}\\
&Y\in\mc{C}_{n+1}^*. && \label{eq: uc1_cpp_profitable_4}
\end{alignat}
\end{subequations}
Observe that this is similar to the CPP \eqref{eq: uc1_cpp1}, but with additional terms multiplying $q_g$ in the objective and constraints. Note that \eqref{eq: uc1_cpp_profitable} includes both $p_{gt}$, a variable, and $p_{gt}^*$, part of the solution to $\uc^\cpp$.{\cgreen (Cheng: Merve, I think keeping (23f) is better, to clearly show that this is a conic program.}

%The former is a variable while the latter is a constant from constraint \eqref{eq: uc1_cop_profitable_1}.})}

The CPP \eqref{eq: uc1_cpp_profitable} is feasible because we recover $\uc^\cpp$ by setting all $q_g$ to zero. It is bounded due to the equality \eqref{eq: uc1_cpp_profitable_0}, and capacity constraints \eqref{eq: uc1_cpp1_lim1} and \eqref{eq: uc1_cpp1_lim2}, which bound $p_{gt}$. If the problem has an interior, then its dual, \eqref{eq: uc1_cop_profitable}, is feasible. We therefore expect the optimization for RCDP to be feasible whenever the optimization for CDP is feasible. This reasoning leads us to the following proposition:
\begin{proposition}
The RCDP problem \eqref{eq: uc1_cop_profitable} is feasible if its dual, \eqref{eq: uc1_cpp_profitable}, has an interior.
\end{proposition}

%As a final note for the application of COP duality on nonconvex market, we would like to mention that even though our CDP schemes are derived for UC problems, it is easy to adapt them for any nonconvex market problems with both variable and fixed costs. For example, we use the CDP schemes to derive prices for the Scarf's example, a classical nonconvex market problem, in Section \ref{ec: scarf}.
%============SECTION ===========%
\section{Mixed-Binary Quadratic Games}\label{ch: app_game}
In this section, we use copositive duality to characterize the equilibria of MBQGs. In an MBQG, each player solves an optimization of the form $\mc{P}^\bqp$, which are coupled through the objectives, but not the constraints. The binary decisions preclude the direct use of existence results for continuous games, and the use of the KKT conditions for obtaining equilibria. We surmount these issues by converting each players MBQP to a CPP, as described in Section \ref{ch: new_results}. We give conditions for existence and uniqueness in Section \ref{subch: pne_exist}, and compute PNE using the KKT conditions in Section \ref{subch: compute_ne}).

%In this section we apply the COP duality concept to MBQ games, which is a special type of IPGs. An MBQ game is defined as a game where each player faces an MBQP in the form of $\mc{P}^\bqp$. Because of the binary variables in $\mc{P}^\bqp$, the PNE existence result for games with convex strategy set cannot be directly used for MBQ games. Also, we cannot apply KKT conditions for finding the NE as $\mc{P}^\bqp$ does not have strong duality. We overcome those difficulties by transforming discrete MBQ games to convex completely positive games (Section \ref{ch: reduction}), then utilize this relationship to propose PNE existence and uniqueness theorems (Section \ref{subch: pne_exist}), as well as KKT conditions for computing the PNE(Section \ref{subch: compute_ne}).
%In this section, we prove some theoretical results for general MBQ games with the novel tool of copositive programming duality. %As we mentioned in Section \ref{ch: app_pricing}, the problem where each generator tries to maximize the profit under the pricing mechanism $\pi^\so$ can be viewed as a MBQ game.

We study an $n$-person MBQG, $\mc{G}^\bq = \langle\mc{I}, (\mcXi)_{i\in\mc{I}}, (\xith)_{i\in\mc{I}}\rangle$, where $\mc{I}$ is the set of indices for the players and $|\mc{I}| = n$, $\mcXi$ is the strategy set of player $i$, and $\xith\in\mcXi$ is the $n_i$-dimensional decision vector of player $i$, which contains both continuous and binary variables. Let $\mcXni$ and $\xni$ denote the strategy sets and strategies of all players except $i$.

Player $i$ faces the following MBQP:
\begin{subequations}\label{eq: ip_game}
\begin{alignat}{4}
\mc{P}^\bqp_i(\xni) : \min ~~& f_i(\xith, \xni)\label{eq: ip_game_obj}\\
\st ~~& \aijtop\xith = \bij, &&\forall j = 1, ..., m_i\label{eq: ip_game_1}\\
%& \aj^{2\top}{\bf x} = b^2_j, &&\forall j = 1, ..., m_2\label{eq: ip_game_2}\\
&x_{ik}\in \{0,1\}, &&\forall k\in\mc{B}_i\label{eq: ip_game_3}\\
&\xith \in \mb{R}_+^{l}.\label{eq: ip_game_4}
\end{alignat}
\end{subequations}
$f_i(\xith, \xni) = \x^\top Q^{(i)}\x + 2 {\bf c}^{(i)\top} {\bf x}$ is the quadratic payoff function of player $i$, $\x$ the vector of all strategies, and $Q^{(i)} \in \mc{S}_{n_i}$ a symmetric matrix. Constraints \eqref{eq: ip_game_1} are linear and independent of the decisions of other players. $\mc{B}_i$ is the subset of indices corresponding to the binary decisions of player $i$.% Let $\feas(\mc{P})$ denote the feasible region of an optimization problem $\mc{P}$. Then in our setup $\feas(\Pith^\bqp(\xni)) = \mc{X}_i, \forall i\in\mc{I}$, because there are only private constraints in each player's problem.

We define a pure-strategy NE (PNE) of $\mc{G}^\bq$ as a vector of actions ${\bf x}^*\in(\mcXi)_{i\in\mc{I}}$ such that for each player $i$: %$\hat{\bf x}$ is the $l_1$-dimensional subvector of ${\bf x}$ that contains all binary variables. Constraints \eqref{eq: ip_game_2} are coupled linear constraints that depends on other players' decisions. 

%To define the NE, we first introduce some more notations. Let's denote $\mcXi = \{{\bf  x}| \eqref{eq: ip_game_1}-\eqref{eq: ip_game_4}\}$, and let $\mc{X} = \mc{X}_1\cap...\cap \mc{X}_n$ be the set of all feasible strategies. Then the GNE of the $n$-person nonconvex quadratic game is given by the point ${\bf x}^*\in(\mcXi)_{i\in\mc{I}}$ such that for each player $i$:
$$f_i(\xstari, \xstarni)\leq f_i(\xith, \xstarni), \forall \xith\in\mcXi,$$
which is equivalently stated
\begin{align}
f_i(\xstari, \xstarni) = \text{opt}(\mc{P}^\bqp_i(\xstarni)).
\end{align}
%i.e., at a PNE player $i$ cannot achieve a better payoff by only changing her own behaviours.

%More generally, define a {\it strategy} $\si$ for player $i$ as a probability assignment to player $i$'s actions $\xia \subseteq \mcXi$, where $a\in\mc{A}_i$ is the index for player $i$'s action in $\si$, and $\mc{A}_i$ is a finite set. Then $\si = \sum_{a \in \mc{A}_i}p_{a}\xia$, where $p_a$ is the probability for action $\xia$, $\sum_{a\in\mc{A}_i} p_a= 1$. The vector $(\s^*_1, ...,\s^*_{\mc{I}})$ is an NE if for each player $i$:
%\begin{align}
%\sum_{a\in\mc{A}^*_i}\sum_{\ap\in\mc{A}^*_{-i}} p_a p_\ap f_i(\x^*_{ia}, {\bf x}^*_{-i\ap})\leq \sum_{a\in\mc{A}_i}\sum_{\ap\in\mc{A}^*_{-i}} p_a p_\ap f_i (\x_{ia}, {\bf x}^*_{-i \ap}), \forall \mc{A}_i\subseteq\mcXi
%\end{align}
%where $\ap = a_{[-i]}$ is a vector for actions of players other than $i$, and $p_\ap = \prod_{j\in\mc{I}\sm i} p_{j a_j}$.
%
%An NE is a PNE if for all players the set $\mc{A}_i$ is a singleton. If the set $\mc{A}_i$ may contain more than one action, then the NE is called a mixed-strategy NE (MNE).
%---%
\subsection{Reformulation in terms of CPP}\label{ch: reduction}
We reformulate $\mc{G}^\bq$ in terms of CPP, and show how the PNE of one can be obtained from the other, and vice versa. Throughout this section, we use the CPP reformulation $\mc{P}_r^\cpp$ because it has several advantages over $\mc{P}_o^\cpp$. For this reason we assume that \eqref{a: alpha} holds throughout. However, we could in principle derive all of the results in this section using $\mc{P}_o^\cpp$, in which case \eqref{a: alpha} need not hold.

We denote the game $\mc{G}^\cpp= \langle\mc{I}, (\mcXip)_{i\in\mc{I}}, (\xith, \Xith)_{i\in\mc{I}}\rangle$, where $\mcXip$ is the strategy set of player $i$. Player $i$ solves:
%We reformulate $\mc{P}^\bqp_i$ to a CPP in the form of $\mc{P}_r^\cpp$ \eqref{eq: cpp_reform}: assume problem $\mc{P}^\bqp_i(\xni)$ satisfies property \eqref{a: alpha}, and denote the $\pmb\alpha$ in property \eqref{a: alpha} for $\mc{P}^\bqp_i(\xni)$ as $\alphai$, then problem $\mc{P}^\bqp_i$ is equivalent to the following CPP:
\begin{subequations}\label{eq: cpp_game}
\begin{alignat}{4}
\mc{P}^\cpp_i(\xni) : \min ~~&\tr(Q_{ii}^{(i)}\Xith) + 2\xnitop Q^{(i)}_{-i,i} \xith + \xnitop \Qi_{-i,-i} \xni + 2\ci {\bf x}\label{eq: cpp_game_obj}\\
\st ~~& \aijtop\xith = \bij &&\forall j = 1, ..., m_i\label{eq: cpp_game_1}\\
& \aijtop \Xith\aij = b_j^{(i)2} &&\forall j = 1, ..., m_i\label{eq: cpp_game_2}\\
& x_{ik} = X_{i, kk} &&\forall k\in\Bi\label{eq: cpp_game_3}\\
& x_{il} = \tr(\frac{\alphai \eltop + \el \alphaitop}{2} \Xith) && l = 1,...,n_i\label{eq: cpp_game_4}\\
%&{\bf x} \in \mb{R}_+^{l}\label{eq: cpp_game_5}\\
& \Xith\in\mc{C}_{n_i}^*. \label{eq: cpp_game_5}
\end{alignat}
\end{subequations}
% === Proposition ====
%\proof{Proof.}
%The objective function of $\Pith^\bqp(\xni)$ can be decomposed in terms of $\xith$ and $\xni$: 
%\begin{align*}
%f_i(\xith, \xni) &= \x^\top \Qi \x + \ci\x \\
%& = \xitop \Qi_{ii}\xith + 2\xnitop Q^{(i)}_{-i,i} \xith + \xnitop \Qi_{-i,-i} \xni + 2\ci_i \xith + 2\ci_{-i}\xni \\
%& = \xitop \Qi_{ii}\xith + 2(\xnitop Q^{(i)}_{-i,i} + \ci_{i}) \xith + \xnitop \Qi_{-i,-i} \xni + 2\ci_{-i}\xni.
%\end{align*}
%
%$\xni$ is treated as a constant vector in $\mc{P}^\bqp_i(\xni)$. Therefore, via Proposition \ref{th: reform_game}, $\mc{P}^\bqp_i(\xni)$ is equivalent to the following CPP:
%\begin{align*}
%\min ~~&\tr(Q_{ii}^{(i)}\Xith) + 2(\xnitop Q^{(i)}_{-i,i} + \ci_{i}) \xith + \xnitop \Qi_{-i,-i} \xni + 2\ci_{-i}\xni\\
%\st ~~& \aijtop\xith = \bij &&\forall j = 1, ..., m_i\\
%& \aijtop \Xith \aij = b_j^{(i)2} &&\forall j = 1, ..., m_i\\
%& x_{ik} = X_{i, kk} &&\forall k\in\Bi\\
%&\xith = \Xith \alphai\\
%& \Xith\in\mc{C}^*
%\end{align*}
%
%Rearrange the terms in the objective, and we obtain $\mc{P}^\cpp_i(\xni)$.
%\Halmos\endproof
% === End of Proposition ====
Note that $\xith$ and $X_i$ are the only variables in $\mc{P}^\cpp_i(\xni)$, and $\xni$ is treated as given. $\alphai$ is defined for $\mc{P}^\bqp_i$ as in \eqref{a: alpha}.

%We introduce a type of $n$-player {\it CP game} $\mc{G}^\cpp= \langle\mc{I}, (\mcXip)_{i\in\mc{I}}, (\xith, \Xith)_{i\in\mc{I}}\rangle$, where $\mcXip$ represents the strategy set of player $i$. In this game, each player $i$ solves a CPP $\Pith^\cpp(\xni)$.

Let $F_i(\xith, \Xith, \xni)$ denote the objective function of $\Pith^\cpp(\xni)$. A PNE of $\mc{G}^\cpp$ is a set of strategies, $(\mathbf{x}^*_i, X^*_i)_{i\in\mc{I}}\in(\mcXip)_{i\in\mc{I}}$, such that for each player $i$:%, $\mcXip = \{(\mathbf{x}, X)|\eqref{eq: cpp_game_1} - \eqref{eq: cpp_game_5}\}$, and $\mc{X}^' = \mc{X}_1^'\cap...\cap\mc{X}_n^'$.  
\begin{align}
F_i(\xstari, \Xstari, \xstarni) = \text{opt}(\mc{P}^{\text{CPP}}_i(\xstarni)).
\end{align}
%i.e., with the decisions of other players fixed at $\xstarni$, $(\xstari, \Xstari)$ is the optimal solution for $\mc{P}^\cpp_i(\xni)$.
%where
%\begin{align*}
%\mc{P}^{\text{CPP}}_i(\xstarni) : \min_{\xith\in\mcXi^'} ~~&F_i(\xith, \xstarni)
%%\st ~~&X_{qq} = x_q^{*2}~~ \forall q\in\mc{D}_i
%\end{align*}
%with $\mc{D}_i\in\mb{R}^{(n-1)\times l}$ being the index set of variables in  $x_{-i}$. 
%\begin{definition} A CPP game is a game where each player solves an optimization problem over a completely positive strategy set.
%\end{definition}

%We define a special type of CPP game $\mc{G}^{\text{CPP}}$, where each player $i$ solves the optimization problem $\mc{P}^{\text{CPP}}_i$. Let $F_i(X, x_i, x_{-i}) := Q\cdot X + 2 {\bf c}^\top {\bf x}$ denote the objective of $\mc{P}^{\text{CPP}}_i$. Then a GNE of the CPP game $\mc{G}^{\text{CPP}}$ is given by the tuple $(X^*, x_i^*, x_{-i}^*)\in\mc{X}^'$ such that for each player $i$: 
%\begin{align}
%F_i(X^*, x_i^*, x_{-i}^*) = \min_{(X, x_i, x_{-i}^*)\in\mcXi^'} F_i(X, x_i, x_{-i}^*)
%\end{align}

With our definition of the CP game, we can transform any MBQ game $\mc{G}^\bq$ to a CP game $\mc{G}^\cpp$. It remains to show the relationship between the Nash equilibria of those two types of games, which is the goal of Theorem \ref{th: games_equiv}: %, due to the equivalence between $\mc{P}^\bqp_i(\xni)$ and $\mc{P}^\cpp_i(\xni)$  (supposing property \eqref{a: alpha} is satisfied)
% === Theorem ====
\begin{theorem}\label{th: games_equiv}
Let $\mathbf{x}^*$ be a PNE of $\mc{G}^\bq$. Then $(\xstari, \xstari \xstaritop)_{i\in\mc{I}}$ is a PNE of $\mc{G}^\cpp$. 

Conversely, if $(\xstari, \Xstari)_{i\in\mc{I}}$ is a PNE of $\mc{G}^\cpp$, and if $(\Qi_{ii}\succeq 0)_{i\in\mc{I}}$, $(\xstarik\in\{0,1\}, \forall k\in\mc{B}_i)_{i\in\mc{I}}$, then $\mathbf{x}^*$ is a PNE of $\mc{G}^\bq$. %then $\mathbf{x}^*$ is an MNE of $\mc{G}^\bq$. A
\end{theorem}
% === End of Theorem ====
{\it Remark. }The requirement $(\xstarik\in\{0,1\}, \forall k\in\mc{B}_i)_{i\in\mc{I}}$ is important for ensuring that a PNE of $\G^\cp$ can be projected to a PNE of $\G^\bq$. In fact, we can replace this requirement with the (possibly more restrictive) condition that the matrix $\begin{bmatrix}
1 & \x^{*\top}_i\\
\xstari & \Xstari
\end{bmatrix}$ being rank-1 feasible for $\mc{P}^\cpp_i(\xni), \forall i\in\mc{I}$, which is similar to the rank-1 feasible condition for recovering an NE from the SDP relaxation of an NE problem in \cite{ahmadi2020semidefinite}. {\cred In fact, it can be easily proved that if 
$\begin{bmatrix}
1 & \xitop\\
\xith & \Xith
\end{bmatrix}$ is a rank-1 feasible solution for $\mc{P}^\cpp_i(\xni)$, then $x^{k}_i\in\{0,1\}, \forall k\in\mc{B}_i$} {\cgreen (Cheng: Josh said this result is standard so no need to prove it.)}
%The following proposition shows the relationship between those two requirements:
%% ===Proposition ====
%\begin{proposition}\label{th: rank_one_equiv}
%Let $(\xith, \Xith)$ be a feasible solution for $\mc{P}^\cpp_i(\xni)$. If 
%$Y_i =\begin{bmatrix}
%1 & \xitop\\
%\xith & \Xith
%\end{bmatrix}$ is a rank-1 feasible solution for $\mc{P}^\cpp_i(\xni)$, then $x^{k}_i\in\{0,1\}, \forall k\in\mc{B}_i$.
%\end{proposition}
%\proof{Proof.}
%{\cred Merve: $Y_i = v w^top$, change the proof accordingly. Explain which constraint X_kk=x_k comes from}
%If $Y_i$ is rank-1 feasible, there exist vectors $\mathbf{w}$ and $\mathbf{v}$ such that $Y_{i} =\mathbf{v}^{\top }\mathbf{w}$. Let $\mathbf{v} \ =\ \left[ v_{1} ,\ \mathbf{v}^{\top }_{2}\right]^{\top }$, $\mathbf{w} \ =\ \left[ w_{1} ,\ \mathbf{w}^{\top }_{2}\right]^{\top }$, and rewrite the rank-1 equation in blocks, we have:
%\begin{align*}
%&\begin{bmatrix}
%1 & \mathbf{x}^{\top }_{i}\\
%\mathbf{x}_{i} & X_{i}
%\end{bmatrix} \ =\ \left[ v_{1} ,\ \mathbf{v}^{\top }_{2}\right]\begin{bmatrix}
%w_{1}\\
%\ \mathbf{w}_{2}
%\end{bmatrix} =\begin{bmatrix}
%v_{1} w_{1} & w_{1} \ \mathbf{v}^{\top }_{2}\\
%v_{1} \ \mathbf{w}_{2} & \mathbf{v}^{\top }_{2}\mathbf{w}_{2}
%\end{bmatrix}\\
%\Rightarrow~&\mathbf{ x}_i \mathbf{x}^{\top }_{i} =(w_{1} \ \mathbf{v}_{2}^{\top }) ( v_{1} \ \mathbf{w}_{2}) =w_{1} v_{1} \cdot \mathbf{v}^{\top }_{2}\mathbf{w}_{2} =\mathbf{v}^{\top }_{2}\mathbf{w}_{2} =X_{i}\\
%\Rightarrow~&x_{ik}^2 =X_{i,kk} =x_{ik}, \forall k\in\mc{B}_i\\
%\Rightarrow~&x_{ik}\in\{0,1\}, \forall k\in\mc{B}_i
%\end{align*}
%\Halmos\endproof 
%% ===End of Proposition ====

Therefore the second half of Theorem \ref{th: games_equiv} can also be replaced with the following (more restrictive) proposition:
% === Proposition  ====
\begin{proposition}\label{th: games_equiv2}
If $(\xstari, \Xstari)_{i\in\mc{I}}$ is a PNE of $\mc{G}^\cpp$, and if $(\Qi_{ii}\succeq 0)_{i\in\mc{I}}$, and each one of the optimization problems $(\Pith^\bqp(\xstarni))_{i\in\mc{I}}$ has a unique optimal solution, then $\mathbf{x}^*$ is a PNE of $\mc{G}^\bq$.
\end{proposition}
% === End of Proposition  ====

This proposition is true because when $\Pith^\bqp(\xstarni)$ has a unique optimal solution, the solution $\xstari$, which is in the convex hull of $\Pith^\bqp(\xstarni)$'s optimal solutions, must be feasible for  $\Pith^\bqp(\xstarni)$. Then we can follow a similar proof as in Theorem \ref{th: games_equiv} to show that $\mathbf{x}^*$ is a PNE of $\mc{G}^\bq$.
%Proposition \ref{th: games_equiv2} is more restrictive than the second half of Theorem \ref{th: games_equiv}, as when $(\Pith^\bqp(\xstarni))_{i\in\mc{I}}$ have unique optimal solutions, $(\xstari, \Xstari)_{i\in\mc{I}}$ must satisfy $(\xstarik\in\{0,1\}, \forall k\in\mc{B}_i)_{i\in\mc{I}}$. The reverse, however, is not necessarily true.
%----%
\subsection{Existence and Uniqueness of PNE in $\G^\bq$}\label{subch: pne_exist}
We first prove that PNE for $\mc{G}^\bq$ exists with some conventional assumptions. %We also provide conditions for the NE of the game $\mc{G}^\bq$ to be unique.
To prove the existence of NE in $\G^\bq$, we first give Proposition \ref{th: exist_cpp} for the existence of PNE in a CP game $\mc{G}^\cpp$. {\cred This proposition is a straightforward result from the classical PNE existence condition for games with convex strategy sets \citep{debreu1952social, glicksberg1952further, fan1952fixed}, as $\mc{P}^\bqp_i(\xni)$ has a convex feasible region and a linear objective function. }
% === Proposition ====
\begin{proposition}\label{th: exist_cpp}
For each $\mc{P}^\cpp_i(\xni), \forall i = 1,...,n$, if $\mcXip$ is compact, then PNE exists for $\mc{G}^\cpp$. % and $Q \succeq 0$
\end{proposition}
%\proof{Proof.}
%We use the following well-known existence theorem for PNE (see \citep{debreu1952social, glicksberg1952further, fan1952fixed}, for example): For every concave $n$-person game where the strategy set of a player $i$'s maximization problem is convex and compact, and the payoff function is continuous on all players' strategies and concave (convex for minimization) for player i's strategies, then there exists at least one PNE point. 
%%
%%By Theorem 1 of \cite{rosen1965existence}, for every concave $n$-person game, where the strategy set of a player's maximization problem is convex, closed, and bounded, and the objective is continuous on all players' strategies and concave (convex for minimization) for current player's strategies, then there exists at least one pure NE point. {\cgreen (page 20 of \url{https://ocw.mit.edu/courses/electrical-engineering-and-computer-science/6-254-game-theory-with-engineering-applications-spring-2010/lecture-notes/MIT6_254S10_lec05.pdf} uses another theorem (Debreu, Glicksberg, Fan) for this result. Do we need to use that one? seems more formal.)}
%
%In our case, the feasible region $\mcXip$ of $\mc{P}^\cpp_i$ is convex because there are only linear and conic constraints in $\mc{P}^\cpp_i$. We also assumed $\mcXip$ to be compact. The objective of $\mc{P}^\cpp_i$ is linear thus convex on player i's strategies $\xith$ and $\Xith$. It is also continuous for $\x$ and $\Xith$. Thus, $\mc{G}^\cpp$ satisfy all the conditions for the existence of the PNE in a concave $n$-person game. %, which means it has at least one NE point.%In our problem, with $Q\succeq 0$, we ensure
%\Halmos\endproof

To prove the existence of NE in $\G^\bq$, we also need the following lemma for relating the compactness of feasible regions $\mcXi$ and $\mcXip$: 
% === Lemma ====
\begin{lemma}\label{th: equiv_compact}
If $\mcXi$ is compact, then $\mcXip$ is also compact.
\end{lemma}
% === End of Lemma ====

Now we provide a sufficient condition for the existence of PNE in $\G^\bq$:
% === Theorem ====
\begin{theorem}\label{th: exist_qip}
{\bf (Existence of PNE)} In an MBQ game $\mc{G}^\bq$ for each player's optimization problem $\Pith^{\bqp}(\xni)$, if

(i) Property \eqref{a: alpha} is satisfied,

(ii) $\mcXi$ is compact,\\
then the corresponding CP game $\mc{G}^\cpp$ has at least one PNE. Additionally, if

(iii) $\Qi_{ii}\succeq 0$, and

(iv) there exists a PNE $(\xstari, \Xstari)_{i\in\mc{I}}$ for $\mc{G}^\cpp$ that satisfies $(\xstarik\in\{0,1\}, \forall k\in\mc{B}_i)_{i\in\mc{I}}$,\\
%(iv) If the corresponding CP game $\mc{G}^\cpp$ has at least one PNE, then there exists a PNE $(\xstari, \Xstari)_{i\in\mc{I}}$ for $\mc{G}^\cpp$ that satisfies $(\xstarik\in\{0,1\}, \forall k\in\mc{B}_i)_{i\in\mc{I}}$,\\
%(iv) asseume $\mc{G}^\bq$ can be reformulated to a corresponding CP game $\mc{G}^\cpp$, and assume $\mc{G}^\cpp$ has at least one NE, then $\xith^{k*}\in\{0,1\}^{|\mc{B}_i|}, \forall k\in\mc{B}_i$,\\
then PNE exists for the $\mc{G}^\bq$. 
%{\cgreen (This might be wrong. Zero-sum game does not have pure-strategy NE...But zero-sum game does not have convex objective function for all players. $\rightarrow$ We actually do not have restrictions on the convexity of crossed terms.)}%still, if we'd like to reformulate bimatrix game with COP, we can.-- 
\end{theorem}
% === End of Theorem ====

If condition (iv) is not satisfied, and $\G^\cp$ does not have any PNE that satisfies $(\xstarik\in\{0,1\}, \forall k\in\mc{B}_i)_{i\in\mc{I}}$, then $\G^\bq$ does not have any PNE, as stated in the following corollary:
% === Corollary ====
\begin{corollary}\label{th: exist_qip_2}
Assume the optimization problems of $\G^\bq$ satisfy conditions (i) - (iii) in Theorem \ref{th: exist_qip}. If there does not exists a PNE of the corresponding $\G^\cp$ that satisfy condition (iv), then $\G^\bq$ does not have any PNE. %and its corresponding CPP game $\G^\cp$ 
\end{corollary}
%\proof{Proof.}
%\Halmos\endproof
% === End of Corollary ====

Corollary \ref{th: exist_qip_2} is a straightforward result of Theorems \ref{th: games_equiv}: assume for the sake of contradiction that $\G^\bq$ has a PNE $\xstar$, then $(\xstari, \xstari \x_i^{*\top})_{i\in\mc{I}}$ is a PNE for $\G^\cp$ that satisfies (iv), which is a contradiction.

%=== We do not have uniqueness results because the objective of CPP game is linear ====
%To get the uniqueness result for MBQ games, we need to introduce the concept of {\it diagonally strictly convex}:
%
%The uniqueness result for convex games can be straightforwardly extended to MBQ games, as shown by the following theorem:
%
%\begin{theorem}\label{th: unique_qip}
%{\bf (Uniqueness of NE)} In an MBQ game $\mc{G}^\bq$ for each player's optimization problem $\Pith^{\bqp}(\xni)$, if conditions (i)-(iv) from Theorem \ref{th: exist_qip} are true, and additionally assume
%
%(v) $(F_i(\xith, \Xith, \xni))_{i\in\mc{I}}$ is diagonally strictly convex,\\
%then $\G^\bq$ has a unique pure strategy NE. 
%%{\cred If QIP is compact and satisfies assumption (A), then QIP game should have unique GNE when CPP game have unique GNE. Use the property that every optimal solution $x^*$ corresponds to an optimal solution $(x^*, x^* x^{*\top})$\sout{Use corollary 2.5 from Burer.}}
%\end{theorem}
%\proof{Proof.}
%Since conditions (i)-(iv) are satisfied, by Theorem \ref{th: exist_qip} $\G^\bq$ and its corresponding $\G^\cp$ both have pure strategy NE. With the additional condition (v), $\G^\cp$ should have a unique NE \citep{rosen1965existence}, which we denote by $(\xstari, \Xstari)_{i\in\mc{I}}$. By Theorem \ref{th: exist_qip}, $\xstar$ is an NE for $\G^\bq$. If this is not the unique NE of $\G^\bq$, suppose there exists $\hatxstar \neq \xstar$ that is also an NE of $\G^\bq$, then $(\hatxstar_i, \hatxstar_i \hat{\mathbf{x}}^{*\top}_i)_{i\in\mc{I}} \neq (\xstari, \Xstari)_{i\in\mc{I}}$ is an NE for $\G^\cp$, which is a contradiction.
%%Since condition (iii') implies (iii) and conditions (i), (ii) and (iv) are satisfied, by Theorem \ref{th: exist_qip} $\G^\bq$ and its corresponding $\G^\cp$ both have pure strategy NEs. 
%%Let $(\xstari, X^*_I)_{i\in\mc{I}}$ be an NE of $\G^\cp$, then for each player $i$, $(\xstari, X^*_i)$ is an optimal solution to $\Pith^\cpp(\xstarni)$. Since $\mcXip$ is nonempty, closed (as it is compact) and convex, and $F_i(\xstari, \Xstari, \xstarni)$ is strictly convex (as $\Qi_{ii}\succ 0$), $\Pith^\cpp(\xstarni)$ has a unique solution \citep{nedich2008}. Therefore, 
%\Halmos\endproof

Using Proposition \ref{th: games_equiv2}, the condition (iv) in Theorem \ref{th: exist_qip} can also be replaced with the requirement that the optimization problems in $\G^\bq$ all have unique optimal solutions, since this requirement also ensures that a PNE of $\G^\cp$ can be converted to a PNE of $\G^\bq$. It is worth noting that a similar requirement is proposed for the existence of PNE in two-person discrete games, which is a special type of MBQ game, by \cite{mallick2011existence}. In that paper the author proves for a two-person discrete game, if both players have unique best responses and if a condition called Minimal Acyclicity is satisfied, then the PNE must exists.

{\cred We next present conditions for the uniqueness of PNE in MBQ games. We use the concept of {\it diagonally strictly convex (concave)} from \citep{rosen1965existence}: let $\nabla_i u(\x)$ be the gradient of $u$ with respect to $\x$'s subvector, $\x_i$. Additionally, let $u_1,...,u_{|\mc{I}|}$ be a sequence of functions and define $\nabla u(\x) = [\nabla_1 u_1(\x), ..., \nabla_{|\mc{I}|} u_{|\mc{I}|}(\x)]^\top$. Then the payoff functions $(f_1,...,f_{|\mc{I}|})$ are diagonally strictly convex (or concave) for every pair of feasible strategies $\xhat$ and $\xbar$, we have $(\xhat - \xbar)^\top \nabla f(\xbar) + (\xbar - \xhat)^\top \nabla f(\xhat) < 0 ~(\text{or}~>0)$. With this concept, we are ready to present the conditions for ensuring the uniqueness of PNE:  %Similar to the classical result on the uniqueness of PNE for n-person concave games  from \citep{rosen1965existence}.
% === Theorem ==== 
\begin{theorem}\label{th: unique_qip}
{\bf (Uniqueness of PNE)} Suppose an MBQ game $\mc{G}^\bq$ satisfies conditions (i) - (iv) of Theorem \ref{th: exist_qip}. Then $\mc{G}^\bq$ has a corresponding CP game $\mc{G}^\cpp$ and has at least one PNE. Additionally, if

(v) $\Pith^{\cpp}(\xni)$ satisfies certain regularity conditions (e.g., Slater's condition), $\forall i\in\mc{I}$ and

(vi) the payoff functions are diagonally strictly convex, \\ % $(f_1, ..., f_{\mc{I}})$
then $\mc{G}^\bq$ has a unique PNE.
\end{theorem}}
% === End of Theorem ====
%One might be tempted to extend the uniqueness result of concave n-person game \citep{rosen1965existence} to $\G^\cp$ to prove the uniqueness of NE in $\mc{G}^\bq$. However, since the objectives of $\Pith^\cpp(\xni), \forall i\in\mc{I}$ are linear, they cannot meet the sufficient condition which requires the objectives to be diagonally strictly concave (convex for minimization). Therefore, we cannot directly apply the uniqueness property of concave n-person game on $\G^\cp$. For completeness, we include the following proposition to prove that the payoff functions of $\G^\cpp$ are not diagonally strictly convex {\cgreen (Cheng: This result is too strainght-forward, I suggest removing it.)}:
%% === Proposition ====
%\begin{proposition}
%The payoff functions $(F_1(\x_1, X_1, \x_{-1}), ..., F_n(\x_n, X_n, \x_{-n}))$ are not diagonally strictly convex.
%\end{proposition}
%\proof{Proof.}
%Let $\y_i^\top = [\x_i^\top, \vec(\Xith)^\top]$, where $\vec(\Xith) = [X_{i,11}, ...X_{i,n1}, ...,X_{i,1n}, ..., X_{i,nn}]^\top$ is the vectorization of matrix $\Xith$. Denote $\y^\top = [\y_1^\top,...,\y_n^\top]$, and rewrite $F_i(\x_i, \Xith, \x_{-i})$ as $F(\y_i, \y_{-i})$. Finally, let $\nabla F(\y)^\top = [\nabla_1 F(\y_1, \y_{-1})^\top, ..., \nabla_1 F(\y_n, \y_{-n})^\top]$.
%
%If $(F_1(\x_1, X_1, \x_{-1}), ..., F_n(\x_n, X_n, \x_{-n}))$ is diagonally strictly convex, then for $\bar{\y}, \y^* \in(\mcXip)_{i\in\mc{I}}$
%\[(\bar{\y} - \y^*)^\top \nabla F(\y^*) + (\y^* - \bar{\y})^\top \nabla F(\bar{y}) < 0\]
%
%However, because $F(\y_i, \y_{-i})$ is linear in $\y_i$, $\nabla F(\y)= \mathbf{c}$ where $\mathbf{c}$ is a constant. Therefore, 
%\[(\bar{\y} - \y^*)^\top \nabla F(\y^*) + (\y^* - \bar{\y})^\top \nabla F(\bar{y}) = (\bar{\y} - \y^*)^\top \mathbf{c} + (\y^* - \bar{\y})^\top \mathbf{c} = 0,\]
%which is a contradiction.
%\Halmos\endproof
%% === End of Proposition ====
%---%
\subsection{Computing the NE}\label{subch: compute_ne}
The NE of $\G^\cp$ is given by KKT conditions when certain constraint qualification, such as Slater's condition, is met. We write the KKT conditions for $\G^\cp$ explicitly. For all $i\in\mc{I}$, we have:
\begin{subequations}\label{eq: cpgame_kkt}
\begin{alignat}{4}
&\eqref{eq: cpp_game_1} - \eqref{eq: cpp_game_5} \label{eq: cpgame_kkt_1}\\%a
&2Q_{-i,i}^{(i)\top}\xni + 2\mathbf{c}_i-\sum_{j=1}^{m_i} \gamma_{ij} \mathbf{a}^{(i)}_j -\sum_{k\in\mc{B}_i}\delta_{ik} \ek - \sum_{l=1}^{n_i} \xi_{il} \el = 0\label{eq: cpgame_kkt_2} \\% b
& Q_{ii}^{(i)} - \sum_{j = 1}^{m_i} \beta_{ij} \mathbf{a}_j^{(i)} \a^{(i)\top}_j + \sum_{k\in\mc{B}_i}\delta_{ik} \ek \ektop + \sum_{l=1}^{n_i} \xi_{il} \frac{\alphai \eltop + \eltop \alphai}{2} - \Omega_i = 0 \label{eq: cpgame_kkt_3}\\% c
& \Omega_i\in\mc{C}_{n_i} \label{eq: cpgame_kkt_4}\\%d
& \tr(\Omega_i \Xith) = 0 \label{eq: cpgame_kkt_5}%e
\end{alignat}
\end{subequations}
where \eqref{eq: cpgame_kkt_1} are constraints of $\mc{P}^\cpp_i(\xni)$. $\pmb{\gamma}_i$, $\pmb{\beta}_i$, $\pmb{\delta}_i$, $\pmb{\xi}_i$, and $\Omega_i$ are respectively dual variables for \eqref{eq: cpp_game_1} - \eqref{eq: cpp_game_5}. Let $\mc{L}(\xith, \Xith, \xni)$ be the Lagrangian relaxation of $\mc{P}^\cpp_i(\xni)$, i.e.,  
\begin{align*}
\mc{L}(\xith, \Xith, \xni) =  &F_i(\xith, \Xith, \xni) + \sum_{i=1}^{m_i} \Big( \gamma_{ij}(\bij - \aijtop\xith) + \beta_{ij} ((b_j^{(i)})^2 - \aijtop \Xith \aij)\Big)\\
& + \sum_{k\in\mc{B}_i}\delta_{ik}\Big(X_{i, kk} - x_{ik}\Big) + \sum_{l=1}^{n_i} \xi_{il} \Big(\tr(\frac{\alphai \eltop + \eltop \alphai}{2} X_{i}) - x_{il}\Big) + \tr(\Omega_i \Xith).
\end{align*}
Then $\partial\mc{L}(\xith, \Xith, \xni)/\partial \xith = 0$ and $\partial\mc{L}(\xith, \Xith, \xni) / \partial \Xith= 0$ respectively correspond to constraints \eqref{eq: cpgame_kkt_2} and \eqref{eq: cpgame_kkt_3}. Constraint \eqref{eq: cpgame_kkt_4} is necessary because of constraint \eqref{eq: cpp_game_5}, i.e.$\Xith\in\mc{C}_{n_i}^*$. Finally, constraint \eqref{eq: cpgame_kkt_5} enforces complementary slackness. %Note that the KKT conditions above are derived assuming $\mc{P}^\cpp_i(\xni)$ is a minimization problem. If $\mc{P}^\cpp_i(\xni)$ is a maximization problem, then the sign before $\Omega_i$ in \eqref{eq: cpgame_kkt_3} is plus instead of minus.

Because of the existence condition for PNE in Theorem \ref{th: exist_qip}, we can add the following extra constraints to the KKT condition:
\begin{align}\label{eq: kkt_binary}
x_{ik} \in\{0,1\}, \forall k\in\mc{B}_i, i\in\mc{I},
\end{align}
to make sure that the optimal solution is a PNE for $\mc{G}^\bq$ (assuming $Q^{(i)}_{ii} \succeq 0, \forall i\in\mc{I}$ is satisfied). 
%--------%
\subsubsection{Special Case for KKT I: Dimension of $\mcXi$ No More Than 4} 
{\cgreen (Cheng: should we remove this subsection? Not used anywhere. To answer Josh's question: it can't be used for UC as we have additional slack vars and 4 is too small.) }
The KKT conditions \eqref{eq: cpgame_kkt} contain conic constraints $\Xith\in\mc{C}_{n_i}^*$ and $\Omega_i\in\mc{C}_{n_i}$. When the dimensions of $\Xith$ and $\Omega_i$ are no more than 4, we have $\mc{C}_{n_i}^* = \mc{S}_{n_i}^+ \cap \mc{N}_{n_i}$ and $\mc{C}_{n_i} = \mc{S}_{n_i}^+ + \mc{N}_{n_i}$, where $\mc{S}_{n_i}^+$ is the cone for PSD matrices and $\mc{N}_{n_i}$ is the cone of entrywise nonnegative matrices \citep{dur2010copositive}. Therefore, constraints $\Xith\in\mc{C}_{n_i}^*$ and $\Omega_i\in\mc{C}_{n_i}$ can be equivalently replaced by the following constraints when $\dim \Xith\leq 4$:
\begin{subequations}\label{eq: kkt_sdp}
\begin{alignat}{4}
&\Xith \in\mc{S}_{n_i}^+\\
&\Xith \geq 0\\
&\Omega_i - N_i \in\mc{S}_{n_i}^+\\
&N_i \geq 0.
\end{alignat}
\end{subequations}
Then the KKT conditions become a bilinear program over SDP conic constraints. 
%--------%
\subsubsection{Special Case for KKT II: All Variables of $\mc{P}^\bqp_i(\xni)$ are Binary}\label{ch: kkt_special_2}
Another special case for simplifying the KKT conditions is when $|B_i| = l$ in $\mc{P}^\bqp_i(\xni)$ \eqref{eq: ip_game}, $\forall i \in\mc{I}$, i.e. all variables in $\mc{P}^\bqp_i(\xni)$ are binary. Then the KKT conditions \eqref{eq: cpgame_kkt} could be replaced with a MIP problem over copositive cone constraints as follows: for the primal problem constraints, we keep constraints \eqref{eq: cpp_game_1}, and add constraints \eqref{eq: kkt_binary}. Considering the fact that constraints \eqref{eq: cpp_game_2} - \eqref{eq: cpp_game_5} are actually a relaxation of the constraint $\Xith = \xith \xitop$, or $X_{i,j_1, j_2} = x_{i j_1} x_{i, j_2}$, and all variables in $\mc{P}^\bqp_i(\xni)$ are binary, we can replace \eqref{eq: cpp_game_2} - \eqref{eq: cpp_game_5} with the following linear constraints $(\forall i\in\mc{I})$:
\begin{subequations}\label{eq: kkt_mip_comp1}
\begin{alignat}{4}
& X_{i, jj} = x_{ij} && \forall j = 1,...,l \\
& X_{i, j_1 j_2} \leq x_{i j_1} &&\forall j_1\neq j_2; j_1,j_2 = 1,...l \\
& X_{i, j_1 j_2} \leq x_{i j_2}&&\forall j_1\neq j_2; j_1,j_2 = 1,...l \\
& X_{i, j_1 j_2} \geq x_{i j_1} + x_{i j_2} - 1&~~&\forall j_1\neq j_2; j_1,j_2 = 1,...l .
%& X_{i} \in\mc{S}^l_+
\end{alignat}
\end{subequations}

On the dual side, we keep all constraints \eqref{eq: cpgame_kkt_2} - \eqref{eq: cpgame_kkt_4}. For the bilinear complementary slackness constraint \eqref{eq: cpgame_kkt_5}, we linearize it by defining a new matrix $Z_i \in\mc{R}^{l\times l}$, and let $Z_{i, j_1 j_2} = \Omega_{i, j_1 j_2} X_{i, j_1 j_2}$, then this equation can be linearized with big-M constraints. More specifically, constraint \eqref{eq: cpgame_kkt_5} can be replaced with:
\begin{subequations}\label{eq: kkt_mip_comp2}
\begin{alignat}{4}
&\tr(Z) = 0\\
&-m X_{i, j_1 j_2} \leq Z_{i, j_1 j_2} \leq m X_{i, j_1 j_2} &&\forall j_1,j_2 = 1,...,l\\
&\Omega_{i, j_1 j_2} - m (1 - X_{i, j_1 j_2}) \leq Z_{i, j_1 j_2} \leq \Omega_{i, j_1 j_2} + m (1 - X_{i, j_1 j_2})&~~&\forall j_1,j_2 = 1,...,l
\end{alignat}
\end{subequations}
where $m$ is a sufficiently large number. Here we use the fact that elements in $\Xith$ are binary, due to constraints \eqref{eq: kkt_binary} and \eqref{eq: kkt_mip_comp1}.

Now we are ready to put together all the necessary constraints to replace KKT conditions \eqref{eq: cpgame_kkt}, $\forall i\in\mc{I}$:
\begin{subequations}\label{eq: kkt_mip}
\begin{alignat}{4}
&  \aijtop \xith = b_j^{(i)} &~~&\forall j = 1, ..., m_i\\
&\eqref{eq: cpgame_kkt_2}, \eqref{eq: cpgame_kkt_3}, \eqref{eq: kkt_binary}, \eqref{eq: kkt_mip_comp1}, \eqref{eq: kkt_mip_comp2}\\
& \Omega_i\in\mc{C}_{n_i},
\end{alignat}
\end{subequations}
which is a MIP over copositive conic constraints, and can be solved exactly with the cutting plane algorithm in Section \ref{ch: cut_plane} with a MIP solver. If a solution for this system of constraints exists, then it is a PNE for the discrete game $\mc{G}^\bq$. {\cred Note that we cannot solve \eqref{eq: kkt_mip} approximately with SDP solvers such as Mosek, because they cannot solve mixed-integer SDPs.}

As a final note to this section, we would like to mention that with some efforts the results for MBQ games in this section can be extended to mixed-{\it integer} quadratic games that contain general integer decisions, as any bounded general integer variable can be replaced by a set of binary variables.
%---------------------%
\section{Numerical Illustrations}\label{ch: results}%Experimental Results
In this section we present the results of numerical experiments for pricing in nonconvex energy markets and bimatrix games. Section \ref{subsec: electricity_markets_results} includes the results of different pricing schemes for a nonconvex electricity market example. In Section \ref{subsec: bimatrix} we compute the PNE of bimatrix games with the reformulated KKT conditions \eqref{eq: kkt_mip}. We also include a comparison of our COP cutting plane algorithm with other COP algorithms in e-companion Section \ref{ec: max_clique}, and a comparison of different pricing schemes for a classical nonconvex market example called Scarf's example in e-companion Section \ref{ec: scarf}.

Unless otherwise specified, all experiments are implemented in Julia v1.0.5 using the optimization package JuMP.jl v0.20.1. All experiments that solve COPs with our cutting plane algorithm uses CPLEX 12.8. For solving SDP problems in Sections \ref{subsec: electricity_markets_results}, \ref{ec: max_clique}, and \ref{ec: scarf}, we conduct preliminary tests with both Mosek 9.1 and SeDuMi 1.3, then pick the solver which is faster or produces more consistent results. %The computer we use for those experiments runs MacOS and has a 2.3 GHz Intel Core i5 processor and a 16GB RAM.
%-%
%\subsection{COP Algorithms Comparison for Maximum Stable Set}\label{subsec: stable_set}
%To compare our COP cutting plane algorithm with approximation algorithms for COP in literature, we present the results from solving the maximum stable set problem with those algorithms. The maximum stable set problem is a classical example in the literature \citep{de2002approximation} for illustrating the CPP transformation of an MIP. The maximum stable set problem is the problem of finding the maximum stable set number in a graph. It can be formulated as a MIP in the following manner: let $\mc{G} = (\mc{N}, \mc{E})$ be a graph, and $\alpha(\mc{G})$ be the stable set number of $\mc{G}$, then
%\begin{subequations}\label{eq: stable_set_mip}
%\begin{alignat}{4}
%\alpha(G) = \max ~~&\sum_{i=1}^n x_i\\
%\st ~~&x_i+x_j\leq1 &~~&\forall (i,j)\in\mc{E}\\
%&x_i\in\{0,1\} &~~&\forall i = 1,...,n
%\end{alignat}
%\end{subequations}

%The MIP \eqref{eq: stable_set_mip} can be reformulated to a CPP as we demonstrated in this paper. However, in this experiment we choose to use a more concise CPP reformulation from Theorem 2.2 of \cite{de2002approximation}:
%\begin{subequations}\label{eq: stable_set_cpp}
%\begin{alignat}{4}
%\alpha(G) = \max ~~&\tr(ee^\top X)\\
%\st~~&X_{ij} = 0 &~~&\{i, j\}\in \mc{E}\\
%& \tr(X) = 1\\
%&X\in\mc{C}^*
%\end{alignat}
%\end{subequations}
%where $e\in\mb{R}^n$ is a vector of all ones.
%
%Since \eqref{eq: stable_set_cpp} is feasible, bounded, and has an interior \cite{de2002approximation}, strong duality holds for \eqref{eq: stable_set_cpp}, we can also obtain the value of $\alpha(G)$ from its dual COP problem:
%\begin{subequations}\label{eq: stable_set_cop}
%\begin{alignat}{4}
%\alpha(G) = \min ~~&\lambda\\
%\st~~&\lambda I + \sum_{(i,j)\in\mc{E}}y_{ij} E_{ij}  - e e^\top = Y\\
%&Y\in\mc{C}
%\end{alignat}
%\end{subequations}
%where $E_{ij}\in\mb{R}^{n\times n}$ is a matrix with ones at $i^{\textrm{th}}$ row and $j^{\textrm{th}}$ column and  $j^{\textrm{th}}$ row and $i^{\textrm{th}}$ column, and with zeros for all other positions. 
%---%
\subsection{Pricing in Electricity Markets}\label{subsec: electricity_markets_results}
In this section we compare different pricing schemes for the energy market example in Section \ref{ch: app_pricing}. We use the data from the adapted California ISO dataset of \cite{guoageneration}. In our experiments we simplify the dataset so that the cutting plane algorithm can solve the problem to optimality or at least to a reasonable gap. The parameters for the generators we use in our experiments are listed in Table \ref{tab:para_uc}.
\begin{table}[h]
\centering
\caption{Parameters for Generators}
\label{tab:para_uc}
\begin{tabular}{lrrrr}
\hline
                  & \multicolumn{1}{c}{Gen\_1} & \multicolumn{1}{c}{Gen\_2} & \multicolumn{1}{c}{Gen\_3} & \multicolumn{1}{c}{Gen\_4} \\ \hline
$c_g^o$           & 25.0                       & 25.5                       & 44.68                      & 44.68                      \\
$c_g^s$           & 140.94                     & 140.94                     & 86.31                      & 86.31                      \\
$\underline{P}_g$ & 297                        & 238                        & 198                        & 198                        \\
$\overline{P}_g$  & 620                        & 496                        & 620                        & 620                        \\ \hline
\end{tabular}
\end{table}

We start with an instance with 2 generators and 4 hours in the planning horizon (we call it ``the first UC instance"). We assume $d_t = [508, 644, 742, 776]$ and use the generators Gen\_1 and Gen\_2 in Table \ref{tab:para_uc}. To use the cutting plane method to calculate the CDP prices and RCDP prices. Note that for this instance Mosek fails when solving the RCDP problem (returns ``UNKNOWN\_RESULT\_STATUS"), while cutting planes solves it optimally within 282.85 seconds. When using the cutting plane method, we set the bounds of the absolute value for elements in copositive matrices as 1000, and add complementary slackness constraint when solving for CDP prices (see Section \ref{ch: cut_plane}). 

We compare RP, CHP, CDP and RCDP (all pricing schemes are solved to optimality) in the following aspects:

(1) The profits. The profit is calculated by deducting the costs from the total revenue, where the total revenue includes the revenue from uniform and generator-dependent prices, as well as the {\it make-whole} uplift payments (see (3) for details).

(2) The uplift payments from generator-dependent prices.

(3) The make-whole uplift payments. This payment is made when the revenue from electricity prices is not enough to cover the costs. Its value equals exactly the difference between the revenue of costs (``make whole"), so the generators do not operate under a loss.

We present the results in Table \ref{tab:uc_compare_1}, where we compare the profit for generators 1 and 2 (Profit1 and Profit 2, respectively), the total profit (ProfitTotal), the generator-dependent price uplift (GenDepUplift), and the make-whole uplift (MakewholeUplift). 
\begin{table}[h]
\centering
\caption{Comparison of Pricing Schemes for the First UC Instance}
\label{tab:uc_compare_1}
\begin{tabular}{lrrrr}
\hline
                & \multicolumn{1}{c}{RP} & \multicolumn{1}{c}{CHP} & \multicolumn{1}{c}{COP} & \multicolumn{1}{c}{RCDP} \\ \hline
Profit1         & 0                      & 839.45                  & 292.02                  & 1393.55                  \\
Profit2         & 0                      & 0                       & 0                       & 72.13                    \\
ProfitTotal     & 0                      & 839.45                  & 292.02                  & 1465.68                  \\
GenDepUplift    & 497.94                 & 0                       & -201.45                 & 0                        \\
MakewholeUplift & 0                      & 95.25                   & 292.02                  & 0                        \\ \hline
\end{tabular}
\end{table}
In the result, RP gives zero profit for both generators, but relies on the revenue from generator-dependent prices (for generator 2). CHP needs make-whole uplift payment (for generator 2) to fully recover the costs for all generators. Interestingly, COP generates a positive profit for generator 1, and needs a make-whole payment that equals generator 1's profit to cover the costs of generator 2. This demonstrates that CDP is revenue neutral in the whole system, but is not revenue neutral/adequate for individual generators. RCDP is the only pricing scheme that is free from any uplift costs. It also makes sure the generators with a lower cost (generator 1) receives a higher profit, which is desirable and is expected from a market with only uniform prices.

Next, we scale up the instance to include all 4 generators in Table \ref{tab:para_uc}, and 4 hours in the planning horizon (we call it ``the second UC instance"). Now assume $d_t = [1469, 1862, 2144, 2242]$. In Table \ref{tab:uc_compare_2} we again compare the four pricing schemes in ProfitTotal, GenDepUplift, and MakewholeUplift. For this instance, Mosek is unable to solve either CDP nor RCDP, while cutting plane takes a long time to terminate so we terminate it after 3,000 iterations and report the results upon termination. Although the results for CDP and RCDP are not optimal, we observe that the total revenue from uniform and availability prices, as well as the profit, are monotonically decreasing when more cuts are added (see e-companion Section \ref{ec: trend_graph}). This indicates that by adding the cutting planes, the prices are getting closer to more reasonable levels.

When using the cutting plane method, we set the bounds of the absolute value for elements in copositive matrices as 5000. Since we do not solve the problems to optimality, we do not add complementary slackness constraints, as those constraints interfere with the monotonicity of revenue and profit trends.
\begin{table}[h]
\centering
\caption{Comparison of Pricing Schemes for the Second UC Instance}
\label{tab:uc_compare_2}
\begin{tabular}{lrrrr}
\hline
                & \multicolumn{1}{c}{RP} & \multicolumn{1}{c}{CHP} & \multicolumn{1}{c}{COP} & \multicolumn{1}{c}{RCDP} \\ \hline
ProfitTotal     & 86859.52               & 86528.41                &  56560.10                       &129918.33                          \\
GenDepUplift    & 86.31                  & 0                       &  -89354.68                       & 0                         \\
MakewholeUplift & 0                      & 83.44                   &   0                      & 0                         \\ \hline
\end{tabular}
\end{table}

The observation from results of the second instance is similar to the first instance: RCDP is the only pricing schemes that does not generate any uplift costs. It also generates a larger profit than other pricing scheme. Although not solved to optimality, CDP still has a smaller profit than RP and CHP. This is to be expected as strong duality of COP guarantees zero profit. If given more time to run, CDP should eventually have zero profit (not counting the make-whole uplift).

Overall, we believe RCDP is a better choice compared with other three pricing schemes, as it only relies on uniform prices to ensure revenue adequacy. %Plus, the change of RCDP uniform prices with demand levels is not too volatile.
%---%
\subsection{KKT Conditions for Bimatrix Games}\label{subsec: bimatrix}
We illustrate the copositive programming formulation \eqref{eq: kkt_mip} for KKT in Section \ref{ch: kkt_special_2} with bimatrix games. A bimatrix game has two players, players 1 and 2. Each player has $n_i$ strategies to choose from, and we use the binary vector $\x_i\in\{0,1\}^{n_i}$ to denote player $i$'s decision. The elements of $\x_i$ are binary since we only look for a pure strategy. Player $i$ faces the following maximization problem:
\begin{subequations}\label{eq: bimatrix}
\begin{alignat}{4}
\max~~ &\x_1^\top R_i \x_2\label{eq: bimatrix_obj}\\
\st ~~& \sum_{j=1}^{n_i} x_{ij} = 1\label{eq: bimatrix_1}\\
& x_{ij} \in\{0,1\} &~~&\forall j=1,...,n_i
\end{alignat}
\end{subequations}
where $R_i\in\mc{R}^{n_1\times n_2}$ is the payoff matrix. If player 1 plays the $k_1^{\textrm{th}}$ strategy and player 2 plays the $k_2^{\textrm{th}}$ strategy, then the payoff for player $i$ is $R_{i,{k_1 k_2}}$. Thus, \eqref{eq: bimatrix_obj} maximizes the payoff of player $i$. Constraint \eqref{eq: bimatrix_1} ensures that player $i$ can only take one strategy.

The problem \eqref{eq: bimatrix} has all binary variables and only equality constraints. The upper bound of binary variables are implied by the constraint \eqref{eq: bimatrix_1}, so we don't need to add additional constraints for the upper bounds in the CPP reformulation. Moreover, there is no unary quadratic term in the objective, thus $Q^{(i)}_{ii}$ in \eqref{eq: cpp_game_obj} of $\mc{P}_i^\cpp(\xni)$ is a zero matrix, i.e. $Q^{(i)}_{ii}\succeq 0$. Therefore, bimatrix game satisfies the requirements of Section \ref{ch: kkt_special_2}, and we can use the reformed KKT conditions \eqref{eq: kkt_mip} to solve for the PNE of its CP game counterpart, and then recover the PNE of the bimatrix game from the PNE of the CP game. 

We test the KKT conditions on bimatrix games with 2 to 5 strategies. For each number of strategy we test 5 instances. For all instances we use the cutting plane algorithm to solve KKT conditions \eqref{eq: kkt_mip}. To ensure the boundedness of initial master problems, we set an upper bound of 100 for the absolute values of elements in copositive matrices. Our computational results show that those bounds are big enough for obtaining copositive matrices upon termination (i.e. separation problem objectives equal 0).
%We compare the obtained results from our method with the results from the lrsnash bimatrix game solver \citep{avis2010enumeration}, and observe that for all instances our method returns the correct results. 
We ensure the correctness of our results by comparing with the results from the lrsnash bimatrix game solver \citep{avis2010enumeration}. 

In Table \ref{tab: bimtrix} we summarize the performance of our method. For each number of strategies (Num\_strat), we report the average solving time (Num\_time) in seconds, and the average number of iterations (Mean\_num\_iter). All tested instances are solved in 7 seconds and within 90 iterations. 

\begin{table}[h]
\centering
\caption{Performance of KKT Conditions for Bimatrix Games}
\label{tab: bimtrix}
\begin{tabular}{crr}
\hline
Num\_strat & \multicolumn{1}{c}{Mean\_time} & \multicolumn{1}{c}{Mean\_num\_iter} \\ \hline
2          & 1.54                           & 3                                 \\
3          & 1.48                           & 1                                   \\
4          & 2.45                           & 31                                  \\
5          & 4.75                          & 62                                  \\ \hline
\end{tabular}
\end{table}
%--------------------%
\section{Conclusion}
\label{sec:conc}
Our work proposes a general framework of COP duality, which provides a notion of duality for MIPs and MBQPs, as well as a new tool for theoretically and computationally analyzing discrete problems. We specialize this framework in two applications: nonconvex electricity markets and MBQ games. More specifically, for electricity markets, we propose a new pricing scheme for electricity markets using COP duality. This pricing scheme has the potential to be generalized for other nonconvex markets. For MBQ games, we transform them to equivalent CP games, to obtain the existence theorem and KKT conditions for the PNE. We also propose a novel cutting plane algorithm for COPs, and use it to obtain numerical results for the applications.

For future works, it will be interesting to find other applications of our COP duality framework, e.g. other nonconvex economic problems whose convex counterparts use KKT conditions to construct equilibria. It is also interesting to explore the economic interpretation of COP duality. For example, in discrete markets, can we project COP dual prices to the space of original MBQP problems? How can the COP dual prices be interpreted with the terminologies in the literature of indivisibility goods? On the technical side, it will be helpful to find out classes of discrete markets and games whose CPP reformulations always have strong duality, such as in the example of \cite{sayin2019optimal}. Finally, to improve the applicability of COP duality, it is important to improve our cutting plane algorithm, or develop more efficient algorithms to solve COPs. %In discrete games, are there any real-world meanings for the dual strategies of CP games?


